An Exploration of Post-Editing Effectiveness in Text Summarization

Automatic summarization methods are efficient but can suffer from low quality. In comparison, manual summarization is expensive but produces higher quality. Can humans and AI collaborate to improve summarization performance? In similar text generation tasks (e.g., machine translation), human-AI collaboration in the form of "post-editing" AI-generated text reduces human workload and improves the quality of AI output. Therefore, we explored whether post-editing offers advantages in text summarization. Specifically, we conducted an experiment with 72 participants, comparing post-editing provided summaries with manual summarization for summary quality, human efficiency, and user experience on formal (XSum news) and informal (Reddit posts) text. This study sheds valuable insights on when post-editing is useful for text summarization: it helped in some cases (e.g., when participants lacked domain knowledge) but not in others (e.g., when provided summaries include inaccurate information). Participants' different editing strategies and needs for assistance offer implications for future human-AI summarization systems.

==> Vivian 2021 Dataminr Internship Project/sections/conclusion.tex <==
%!TEX root = main.tex

\section{Conclusion}

%\joel{again - be positive, sell the work!  }
\label{sec:conclusion}
%This work is an exploration for research on post-editing in text summarization.
To take advantage of the complimentary strengths of AI---which can produce summaries quickly---and humans---which can write summaries well---we explored how human-AI collaboration (i.e. post-editing) impacts summary quality, human efficiency, and user experience for text summarization. 
%
%This work is an important step toward understanding the benefits and drawbacks of post-editing as opposed to manual text summarization.
%We explored whether post-editing offers advantages for text summarization, opposed to summarizing manually.
% We explored how post-editing as assistance affects summary quality, efficiency, and user experience.
%by conducting the first large-scale experiment with 72 participants who summarized either informal (\datareddit) or formal (\dataxsum) text.
Through the first large-scale study on post-editing for text summarization, we provide valuable insights on the benefits and drawbacks: %the results showed some areas where post-editing can be an attractive option to achieve X Y or Z but we also learned there are some situations where post-editing won't improve things that much (note I am writing informally)}
compared to summarizing manually, post-editing was helpful for formal news articles, where participants lacked domain knowledge, while post-editing was less helpful for informal social media posts, for which the reference TL;DR summaries sometimes included inaccurate information.
%
We also observed differences in participants editing strategies and needs as well as concerns of over reliance, all of which deserve future exploration. 
%
%From further analysis, post-editing helped in cases when participants lacked domain knowledge but did not help when the provided summaries included inaccurate information.
%
%Participants' also had different post-editing strategies---some made many edits to summaries while others made fewer---regardless of the provided summary quality.
%
%Future text summarization systems might consider alternative workflows---e.g., showing summaries before or after users write manually (or not at all)---based on users' preferences and the quality of the provided summaries. 
%
We hope this initial exploration provides a starting point for future research on post-editing in text summarization.
% Our findings suggest that humans have different summarization goals and post-editing assists humans in creating a summary to achieve their goals or cater to a particular audience.
%Finally, we proposed design recommendations for future text summarization systems.
% This initial exploration should provide a starting point for future research on post-editing in text summarization.
% %The results have shown that it can be beneficial to have a human-AI collaboration for text summarization processes.
% %
% While supporting post-editing improved the quality of the provided summaries, it was not always better than simply summarizing manually (without a provided summary for assistance).
% %
% Post-editing helped for the news dataset, when more context was needed, but not for Reddit, likely due to Reddit's low quality provided summaries.

% \joel{conclusion needs to be tightened up and end on a more positive note}

%In certain cases, efficiency is worse than when humans are not provided any assistance.
%An interesting direction would be to conduct studies that understand how humans receive and apply information, thereby improving the process of humans and AI systems working together.

% \alison{cite other similar IML work? anything in MT that does this?}
% \viv{can we leave out this entire paragraph? i think if we want to talk about it we can briefly mention in discussion}\alison{we can move this into discussion}
% While we did not use the post-edited summaries to feedback into the model, such iterative methods could be used to gather more human training data more quickly, creating a tighter interaction loop between human and AI.
% %
% Future work might also explore additional forms of assistance (e.g., autocomplete) or domains (e.g., medical or legal documents).

%For example, post-edited summaries could be used for training purposes and create a tighter interaction loop between human and AI.
%Our work suggests future directions for more human-centered text summarization studies and development of design principles that ensure smooth and effective human-AI collaborations specifically on text summarization processes.


%Prior work in human-AI collaborations have displayed other forms of assistance such as autocompletion.
%Instead of post-editing the provided summary, another option could be to allow autocompletion while the human writes the summary.
%It would be interesting to compare the effects between the two types of AI assistance.

%We conduct the first full-scale study that investigates the effects of implementing AI assistance -- post-editing -- in the text summarization process.
%We conclude that (1) post-editing improves summary quality as compared to the quality of provided summaries; and (2) providing summary as a form of assistance improves the final summary quality to a certain extent as compared to when assistance is not provided. 
%Additionally, regardless of provided AI assistance, user experience neither improves or worsens, suggesting future directions for more human-centered text summarization studies to understand effective human-AI collaboration. 

==> Vivian 2021 Dataminr Internship Project/sections/data_collection.tex <==
\subsection{Phase I: Summary Collection}
\label{sec:summary_collect}
% \alison{this needs a section or introduction before that describes the full study design and goal and rqs, then you can have a section for details on each phase followed by the results section}
% \alison{let's add in the figs soon to get a better idea on clarity and space}
% \alison{instead of saying what we will discuss in this section, summarize this phase here, something like, ``In this phase, participants review documents (either informal or formal) and provide summaries either without any assistance or post-editing either a model generated summary or a human written reference summary''.}
% In this section, we describe how the first phase was conducted and provide details on the methods and approaches.
% In the first phase of the experiment, 
% Participants first read documents (either informal and formal) then write summaries either without any assistance or provided with a model generated summary or a human-written reference summary.
% We provide details on the study design, protocol, and implementation.

%\para{Methods and Approaches}
% \alison{this RQ should come before this (and be broken down into the specific RQs)}

\para{Task, data, and model.}
% \alison{briefly introduce the summarization task here, then talk about the two datasets and the model we implement}
The task is to read a document and summarize the document and each participant summarizes 10 documents.
Informal and formal writing might impact how a human understands the context and formulates the summary. 
We employ the Reddit-TIFU dataset \citep{kim2018abstractive} for informal writing and Extreme Summarization (XSum) dataset \citep{narayan2018don} for formal writing.
% As there are many instances in both datasets, 
We randomly selected 120 
% \ke{shouldn't the final size be 120?} 
instances from the default test set downloaded from Huggingface \footnote{\href{https://huggingface.co/datasets/reddit_tifu}{Reddit-TIFU}, \href{https://huggingface.co/datasets/xsum}{XSum}}.
% \ke{provide a link here}.
As lengthy documents make the task more difficult and short documents make the task easier, we selected instances which length fall between the 25th and 75th percentile.

\begin{table}[t]
    \small
    \centering
    \begin{tabular}{p{0.1\textwidth}p{0.15\textwidth}}
    \toprule
    \multicolumn{2}{c}{Rouge-1/Rouge-2/Rouge-L} \\
    Reddit & 27.99/9.81/22.94\\
    Xsum & 47.60/24.83/39.64 \\
    \bottomrule
    \end{tabular}
    \caption{Pegasus performance on Reddit and Xsum datasets.}
    \label{tb:pegasus_performance}
\end{table}
% \alison{provide more details on Pegasus; how well it works and for what types of data it has been used before; describe more details about pretraining}
% \alison{its not clear from this section what the model is doing; let's merge this with data and talk about the task (summarizing documents)}
We use the Pegasus model \cite{zhang2020pegasus} to generate summaries for the two datasets.
The base model is trained with stochastically sample important sentences and models for respective datasets are finetuned from it.
% The Pegasus model for respective dataset is then finetuned from the base model.
The performance of the models are stated in \tabref{tb:pegasus_performance}.
% To ensure the quality of the generated summaries, they are generated by the Pegasus \cite{zhang2020pegasus} model pretrained on the respective dataset, as provided by Huggingface.
% The same tokenizer is used for both datasets.

% \alison{I suppose we need to say this somewhere}
We built a web application to facilitate the first phase of the experiment and conducted a pilot study before running the full user study.
Read appendix for more details of pilot study.
% \footnote{The web application went through a few rounds of iteration to ensure that the wordings and flow was correct and easy to follow.We did two pilot study sessions, the first was conducted among researchers with 5 users mainly to get feedback on the usability of the web application and the average duration of a session, and the second one was conducted with actual targeted users on Upwork.} 



\para{Study design.}
% \alison{we actually did not use a 2x3. we did two 1x3 experiments (one for each dataset) where the only factor is assistance}
% \alison{we might move this to the intro and shorten if we we're having spaces issues}
The study used a 
% 1 x 3 
between-subjects experimental design, using \textit{AI assistance} as the factor.
% with factors of 
% --none, generated summary, reference-- 
% Given that there are two datasets, totalling to 6 conditions. 
The AI assistance factors are the following:
\begin{enumerate}
    \item \textbf{Manual}. There is no provided assistance.
    \item \textbf{Generated summary}. An AI-generated summary is provided as assistance.
    \item \textbf{Reference}. The ground truth summary provided by the dataset is provided as assistance.
\end{enumerate}
% --Xsum, Reddit-TIFU

% \alison{up to?}

% \subsection{Interface \& User study}
%\subsection{User study method}
% \alison{is this your study method section? perhaps rename}



\para{Participants.}
% \alison{be more specific about the skills we wanted and why we used upwork; talk about how much people were paid here and report on their gender, age, etc.}
We recruited 72 participants in total from the Upwork platform.\footnote{https://www.upwork.com}
% \alison{didn't we pay a bonus as well?} \viv{we didn't pay bonus}
Based on pilot studies, we anticipated the entire process would take 60 minutes and we paid participants \$20.
% \alison{oof we paid too much? does that average time count all the way from instruction to submitting the survey? also need to report standard deviation - we can report on this in the results or data and analysis section instead} \viv{time taken is measured from start till finish}
Each participant session took on average 34 minutes ($SD$=15)
% We used Upwork to recruit more motivated and experienced participants compared to other common crowdworking platforms.
% , such as Mechanical Turk. 
%the task of summarizing text requires certain set of skills and also to ensure certain level of summary quality, 
% Specifically, 
We used Upwork to recruit participants with experience in writing, journalism, or communication to ensure higher quality human-written summaries. 
% Participants were required to be a native or bilingual English speaker, have at least 90\% job success score and possess expertise in one or more of: writing, journalism, and communication.
Participants were asked two pre-task questions, 
% the first question was on 
their familiarity with Reddit and British culture.
% and the second question was on their familiarity with British news and culture.
% If participants answered that they have some experience, 
% assuming that they satisfy the previous criteria mentioned, 
% they would be hired as one of the participants.
Pre-task questions ensure that participants do not work on the task without \textit{any} knowledge of the domain.
% (i.e., Reddit and British news and)
% \alison{explain why we asked for reading test score: (1) selection criteria and (2) ensure similar average score per condition... you might need to describe how condition assignment happened somewhere...}
We also asked participants to report their reading test score based on a website \footnote{https://swiftread.com}.
The reading and comprehension test scores help to (1) eliminate potential participants who do not pay close attention to reading and (2) ensure similar average score per condition.
Lastly, participants were assigned to conditions in a round-robin manner.
% while adhering to similar average reading speed in different conditions.
% For instance, if a participant was assigned to manual in Reddit, the next participant would be assigned to generated summary in Reddit, etc.


% \alison{report the average age and standard deviation}
Participants' varied in age from 18 to 71 (M=32, SD=12) and gender (45 female, 22 male, 3 non-binary, 2 preferred not to disclose).

% \alison{did we ask any other pre-task or qualifying questions?}


% \para{Pilot study.}
% % \alison{this might fit better somewhere else; perhaps earlier?}
% \alison{maybe this is better as a footnote for saving space (you can footnote it when you first mention the pilot)}
% The web application went through a few rounds of iteration to ensure that the wordings and flow was correct and easy to follow.
% We did two pilot study sessions, the first was conducted among researchers with 5 users mainly to get feedback on the usability of the web application and the average duration of a session, and the second one was conducted with actual targeted users on Upwork.


% \para{User study flow.}
\para{Procedure.}
%From pilot studies, we anticipated it would take about an hour to complete the task.
An equal number of participants (36)
% \alison{how many?}
were randomly assigned to each dataset and summarization condition.
During the study, participants completed four phases: (1) instructions, (2) tutorial and practice, (3) summarization task, and (4) post-task survey.
% Participants were paid \$20.
%Using the web application to collect information, participants went through four phases during the study: (1) instructions; (2) tutorial and practice; (3) summarization task; (4) exit survey.
% \alison{is this your protocol section? perhaps rename}
% \alison{let's just very briefly discuss the instructions, tutorial and practice; the important part is the summarization task} \viv{ok sounds good}
During the \textit{tutorial and practice}, participants are taught the criteria of a good summary and how to write a good summary.
We used the same criteria of a good summary as in \citet{stiennon2020learning}.
The participants reviewed two randomly selected documents with a bad and good summary each with individual explanations provided.
% The two documents are randomly selected from the original training set of both Reddit and Xsum.
% Individual explanations are given for each summary provided.
Read appendix for details on each phase.
% \figref{fig:tutorial} shows the criteria of a good summary.



% During the \textit{practice} phase, participants applied what they learned in the tutorial phase and practiced how to write a good summary.
% To refrain from any confusion, the interface in the practice phase is exactly the same as the actual summarization task phase.
% Participants have access to the criteria as guidance.
% % \figref{fig:practice} shows the interface during the practice phase.
% After completing the summary, participants rated their agreement with two or three statements (depending on the assigned condition) about the task.
% % \alison{don't need to detail the measures here (they have their own section), just say they rated their agreement to three statements about the task.. except, how to explain that we don't report on one of these measures?}
% % \viv{can we just leave out the third one?}
% % \alison{yes, since we didn't log or report on it let's leave it off}
% We asked participants to rate their agreement for the following statements: (1) I found it difficult to understand the content of the document; (2) I found it difficult to summarize the document well. 
% % (3) The provided summary was of poor quality.
% % The last statement is only shown to participants who have provided summary or reference as AI assistance.
% % \ke{let's define clearly the conditions at the beginning, like (1) AI model automatically generated summary; (2) reference summary which is provided by dataset; (3) manual, where no summary as assistance provided}.

% During the actual summarization task phase, participants see the exact same interface as they saw in the practice phase.
% Finally, participants They would complete summarizing 10 documents and proceed to answer an exit survey.


% \para{Pilot study.}
% \alison{this might fit better somewhere else; perhaps earlier?}
% The web application went through a few rounds of iteration to ensure that the wordings and flow was correct and easy to follow.
% We did two pilot study sessions, the first was conducted among researchers with 5 users mainly to get feedback on the usability of the web application and the average duration of a session, and the second one was conducted with actual targeted users on Upwork.


\para{Measures.}
\label{para:measures}
% We report on summarization quality, efficiency, and user experience for the summarization task. 
% \alison{summary quality belongs in the second phase discussion but we can forward ref it here}
Summary quality is measured using human evaluation where a summary is rated on four axes: Coherence, Accuracy, Coverage, and Overall, on a scale of 1 to 7 
% (see \secref{sec:summary_evaluate}) 
and ROUGE.
% We also report on summary quality as measured by automatic measures (ROUGE), but such measures do not typically align well with human quality ratings~\cite{}.
%Summary quality is rated by four axes, Coherence, Accuracy, Coverage, and Overall on a 7-point scale from 1 to 7.
%We follow the rating design as written by \citet{stiennon2020learning}.
Efficiency is measured by the amount of time taken to complete writing a summary for each document. 
% As it is not simple to extract summarization time from reading time (as participants might switch back and forth between reading the original document and writing their summaries), we measure the time taken from when the participant receives the original document to when they submit their summary.
% We account for individual reading time differences by ensuring a similar average reading speed, measured by words per minute (WPM), between participants (M=358, SD=).
% \alison{we need to report on average reading score per condition somewhere - perhaps here? or report somewhere else and reference from here}
Finally, we report on three subjective measures related to user experience, collected using 7 point rating scales (from strongly disagree to strongly agree):
task-level task ease, or ``The summarization tasks were difficult.''; 
instance-level task ease, or ``I found it difficult to summarize the article well.''; and, task-level frustration, or ``Performing the summarization tasks was frustrating.''

==> Vivian 2021 Dataminr Internship Project/sections/data_evaluation.tex <==
\subsection{Phase II: Human Evaluation of the Collected Summaries}
\label{sec:summary_evaluate}
% \alison{instead of saying what you will write about in this section, give an overview of the purpose of this Phase and what was done; you can also succinctly introduce the summary types (conditions) here instead of later.}
% In the previous section, we described the process of collecting human written summaries and in this section, we detail the process of evaluating the summaries collected.
% In the second phase of the experiment, 
We hire another set of participants to evaluate the human-written summaries.
% collected during the first phase of the experiment.
% A participant reads a news article or Reddit post and 
A participants evaluates six different summaries written or generated for the same document.
% \alison{might be more clear in a list? }
The six types of summaries are the following: 
\begin{enumerate}
    \item \textbf{Manual}. It was written without assistance.
    \item \textbf{Model-generated}. The provided summary is generated by the Pegasus model.
    \item \textbf{Reference}. The provided summary is from the original dataset.
    \item \textbf{Model-generated + post-edit}. It is written by a human who is shown a model-generated summary.
    \item \textbf{Reference + post-edit.} It is written by a human who is shown a reference summary.
    \item \textbf{Random.} It is generated by randomly selecting two sentences from another dataset. This summary helps to weed out turkers who do not pay attention. Refer to appendix for details.
    % For instance, if the participant sees a Reddit post, the \textit{Random} summary is a summary generated from a news article from the Xsum dataset.
\end{enumerate}

% \subsection{User study}
% \alison{this is not a user study; this is purely a data collecion task to evaluate the summaries collected in Phase I}
% \viv{what is a good subtitle?}


\para{Participants.}
% For the second phase of the experiment, as compared to writing a summary, evaluating a summary is an easier task.
We hire participants from crowdsourcing platform, Amazon Mechanical Turk as evaluating summaries is a relatively easier task.
To ensure quality responses, we only employ turkers who satisfy the following criteria: (1) completed 5000 HITs; (2) 97\% HIT approval rate; (3) Reside in the United States, Australia, and United Kingdom.
We allow duplicate participation given the assumption that users become better at the task if they constantly work on a similar task.
Refer to appendix on how we did quality-control on turkers.

\para{Procedure.}
The participant goes through two phases in this user study: (1) tutorial and attention check; and (2) the task of evaluating summaries.
A tutorial is written at the start of the task to teach the participant how to evaluate a summary.
We included an attention check open-ended question to ensure that the participant read through and understood the tutorial.
% Following \citet{stiennon2020learning}, a summary is rated on four axes: Coherence, Accuracy, Coverage, and Overall, on a scale of 1 to 7.
% Examples are given to ensure that the participant knows what a rating of 1, 4, or 7 look like.
% \figref{fig:rating_table} shows the table that was shown to participants.
To further solidify their understanding, we also included two examples with ratings and explanations.
% \figref{fig:evaluate_examples} shows the two examples taken from the training set of datasets.
Explanations are curated by the researchers and iterated a few times upon getting feedback.
% The attention check question does not disqualify the participant but only allow the participant to proceed to the actual task if only they answered it correctly.

% A participant reads a news article or Reddit post and evaluates six different summaries written for the same post.
% % \alison{might be more clear in a list? }
% The six types of summaries are the following: 
% \begin{enumerate}
%     \item \textbf{Manual}. The summary was written without any form of assistance.
%     \item \textbf{Model-generated}. The provided summary is generated by the Pegasus model.
%     \item \textbf{Reference}. The provided summary is from the original dataset.
%     \item \textbf{Model-generated + post-edit}. The summary is written by a participant who is shown a model-generated summary as provided assistance.
%     \item \textbf{Reference + post-edit} The summary is written by a participant who is shown a reference summary as provided assistance.
%     \item \textbf{Random} The summary is generated by randomly selecting two sentences from the opposite dataset.For instance, if the participant sees a Reddit post, the \textit{Random} summary is a summary generated from a news article from the Xsum dataset.
% \end{enumerate}
% (1) \textit{Manual} where the summary was written without any form of assistance; (2) \textit{Model-generated} summary that is generated by the Pegasus model; (3) \textit{Reference} that is provided with the original dataset; (4) \textit{Model-generated + post-edit} summary that is written by a participant who is shown a model-generated summary as provided assistance; (5) \textit{Reference + post-edit} summary that is written by a participant who is shown a reference summary as provided assistance; and (6) \textit{Random} summary that is generated by randomly selecting two sentences from the opposite dataset.


% \begin{figure}[t]
%   \centering
%     \centering
%     \includegraphics[width=.4\textwidth]{figs/sample-franklin.png}
%   \caption{This shows an example of a random summary for a particular instance from the Reddit-TIFU dataset.}
%   \label{fig:random_summary}
%   \Description{}
% \end{figure}

% \para{The purpose of the \textit{Random} summary.}
% The \textit{Random} summary helps to weed out turkers that do not pay attention and simply click through the rating scales.
% Since the order of the summaries is randomized, the \textit{Random} summary can appear in any position, minimizing the potential of participants not paying sufficient attention to details.
% Given that there are four axes to rating a summary, we eliminate and leave out responses of turkers who do not give a rating of 1 to Coverage and Accuracy.
% Since the \textit{Random} summary is created by using another document from an entirely different dataset, it is fair to assume that the content will not overlap and be inaccurate.
% \figref{fig:random_summary} shows an example of a random summary for post from the Reddit-TIFU article.


% \para{Eliminating the bad apples.}
% % \viv{this is one of our contributions. should we elaborate more on this?}\alison{if it will be a contribution, then yes}
% % \viv{let's discuss with joel}
% We deployed a total of 1200 evaluations (i.e., 120 HITs x 2 datasets x 5 samples) on Mechanical Turk.
% To maintain the integrity of the results, instead of deploying all assignments at once, we split the assignments into 10 batches.
% At the end of a batch deployment, turkers who failed the Random summary check will be blacklisted and not allowed to take accept future HITs in this group. A total of 113 workers completed the 1200 evaluations.


==> Vivian 2021 Dataminr Internship Project/sections/discussion.tex <==
%!TEX root = main.tex

\section{Discussion}

% \joel{when I saw discussion, I thought this was the conclusion but there is actually another page to go.  Is there a reason to make two whole sections?  It seems like we are repeating things ad nauseum from Section 4?  } \alison{the discussion should be a synthesis of the findings with big takeaways - it should be short and not repeat too much of what came before}

% \joel{for the discussion and/or conclusion start off on a positive note:  remind the readers that this is the first large scale study of its kind for summarization etc etc.  and remind the readers why this work is important and interesting, and maybe even a bit hard. Mixed (to me) is not bad because we as a community now have a better understanding of what can work from quantitative and qualitative sides }

%\joel{if we go with the discussion section, let's be clear about what is being discussed.  At times it seems like future work, which is fine, but then let's sign post it that way.  Or it could be "these are three takeaways for the research community on when post editing works / doens;t work}

% \joel{another takeaway - maybe post-editing is effective with certain genres (formal vs. informal)  we could probably make a table with check boxes for all these configurations}


\label{sec:discussion}

This work is the first large-scale study of post-editing for text summarization, providing valuable insights on the benefits and drawbacks.
%
We discuss these, as well as outline future research directions and design recommendations for post-editing summarization systems. Finally, we discuss the limitations of our experiments. 
%This study sheds valuable insights on when post-editing is useful for text summarization


%Our experiments indicate that post-editing is not a one-size-fits-all solution for human-AI text summarization due to participants' different editing strategies and needs for assistance, as well as qualities of the provided summaries.
%
%We relate our findings to prior work, provide design recommendations for text summarization systems, and discuss limitations of this experiment.
%\alison{we mostly talk about findings and design reccs from the system perspective (e.g., how should human-AI text summarization systems be provided; if possible, we should update to give insights for (1) summary collection tasks - should practitioners use manual, post-editing, or some combo? and (2) summary model developers - what qualities should we strive for in ai-generated summaries? which were especially problematic?}\ke{like a iterative active learning process to improve AI (quality) and thus human (efficiency)}
%\alison{another thing we could have done but didn't is to train a model using the post-edited summaries (perhaps even vs. the manual) to see their utility for training; is this something we should even discuss? or ignore?}

\para{Post-editing was useful when domain context is needed.}
%While participants in both datasets commented that the provided summaries were great starting points, the effect of post-editing is more pronounced in \dataxsum as post-editing leads to similar summary quality as manual.
As our participants were not well-versed in the British news content of \dataxsum, the provided summary was ``useful'' as a starting point (as described in qualitative responses), so that they did not have to write from scratch.
This is similar to machine translation literature, which suggests that monolingual editors, despite lacking the knowledge of the other language, can still effectively improve the quality of translation via post-editing~\citep{koehn2010enabling}.
% ~\citep{Plitt2010APT,garcia2010machine}.
%
Beyond post-editing, systems could provide additional support when users lack domain knowledge or context, such as inline web searching to learn about unknown terms or phrases (e.g., the rules of Cricket).  
%On the other hand, the lack of domain knowledge or context reported by many participants suggests the need for additional assistance.
% Many participants in \dataxsum also reported that the lack of domain knowledge implicated their ability to summarize, which reflects similar observations in machine translation literature that 
% As such, there is potential in improving the text summarization process in unfamiliar contexts if further assistance was provided.
%To this, we recommend that future systems include features such as inline web searching to help users understand the unknown.
%For example, with inline web searching, \dataxsum participants would be able to find out the rules of cricket, understand the article and summarize better.
% To resolve the problem of skill transferability, we recommend AI models be designed to learn from summaries written by domain experts.

\para{Post-editing was less useful when the provided summaries were low quality.}
%While some summaries were helpful, others included inaccurate or redundant information, which might confuse users and result in lack of trust. 
%They also commented that it was difficult to match the tone and writing style of the original documents in their summaries, suggesting that the provided summaries did not follow the style and tone of the original document.
%Since an inaccurate summary can not only confuse humans but also make them lose trust in the provided assistance, 
Low quality, particularly inaccurate or incoherent, provided summaries can be confusing and hard to edit, making them less ``useful'' as summarization assistance.
Ideally, such summaries are not provided for post-editing, as manual summarization would be better in those cases.
%
Future systems should explore techniques for determining \textit{whether} to provide a summary or not, based on desired summary qualities.
%Therefore, we recommend that future systems should first filter provided summary by a few criteria before presenting it to humans.
%As matching the tone and writing style is important to preserve the integrity of the document, more than one provided summaries could be provided.
Finally, systems might provide \textit{transparency}, e.g., highlighting the important details in the original text~\citep{lai2019human}.
% \alison{cite?}).
Then users can then decide for themselves whether or not those details are important and the summary should be trusted or ignored.
%Users could choose the best summary, edit to include nuanced details that provided summaries would miss, and make adjustments to the style as prior work in machine translation has shown that manual translations are more preferable in terms of style~\citep{fiederer2009quality}.
%As our work represents an exploration in understanding the benefits and drawbacks of post-editing in text summarization, we call for future research to further explore cases where post-editing is effective.



\para{Post-editing can lead to over-reliance and stifle creativity.}
%Some participants reported that they had the tendency to over rely on the provided summary, which is observed in 
Humans have a tendency to over-rely on AI systems~\cite{bussone2015role,buccinca2021trust}: 
%\joel{is it one word or two words? It's used both ways in this section.  } 
% \alison{cite}
prior work on text generation found users consider the provided text as an ``authority'' and thus feel apprehensive to make significant edits~\citep{bhat2021people}.
%
In our experiment, some participants reported a similar tendency to over-rely on the provided summary or were distracted from writing their own version of the summary; some even developed their own combative strategies: writing their summaries manually first and then referring to the provided assistance.
%
Therefore, future systems might allow different workflows, where summaries are shown before or after manual summarization (or not at all).
%
%Further, allowing users to hide/show a provided summary gives further autonomy.
%Prior work has shown that the autocompletion function encourages creativity in writing~\citep{clark2018creative}, we recommend to include it in future text summarization systems.



\para{Post-editing systems should cater to varied users’ preferences and needs.}
%\alison{this section is a bit weird because it combines from previous; I think the points are important but there might be a better way to organize}
Users have varied summarization strategies and needs for assistance as a result of personal preferences and their experience with the domain. 
%
In our study, some preferred more control over the final summary, making lots of edits, while others made fewer edits, and a few did not use the provided summaries at all.
%
These differences in writing style (and their effects on post-editing in text summarization) are also noted in prior work~\citep{moramarco2021preliminary}.
%
Therefore, systems should give users control over the assistance they receive and alternative workflows, based on their preferences and needs. 

Users' needs also vary by their target audience; users might desire summaries that are longer or shorter, or more formal or informal based on who they expect will read them.
%
Post-editing can help, allowing users to tailor summaries to different audiences with the same underlying content.
%
Future post-editing systems might provide multiple summary options, with diverse content and/or style, from which users can choose.

%Beyond the aforementioned design recommendations. %are applicable to design a system that caters to users' preferences.
%For users who preferred having control over the final summary, they could hide the provided summary and/or turn on the autocomplete function that suggests what to write while summarizing.
%Providing more than one summary with diverse content and style also enables human to learn, select and edit the best option.
%As users may have different behaviors in different domains, further experiments with actual users in realistic settings are necessary to inform the design of future systems.


 %\joel{I agree with Alison's comments.  }
%\joel{However, this isn't a takeway like the preceding paragraph sections are.  It's a separate section and should be noted as such.  I believe Limitations of this Study might be a better title and make its own subsection?  Right now this whole section seems like a grab bag of different thoughts which need to be organized.  }\alison{keeping it as a para for space (but we explain at the top of the discussion that there will be a limitations section}
%\alison{give some examples of the factors we couldn't control for}
%We controlled for reading speed, ensuring a similar average reading speed between all conditions, while given the participant size (12) per condition (although much larger than prior work), we are unable to control all potential confounding factors that could have possibly impacted our results.
%While we controlled the reading speed by ensuring that the participants in different conditions had similar reading speed, there are other factors that are not within our control.
%\alison{what is the recommendation here? what would be manipulated with A/B testing; why is this better?}
%For future work, it is recommended to perform a large-scale A/B testing experiment in production environment.
\para{Limitations.}
We note possible limitations of our results due to the length and nature of the task: participants only interacted with the summarization system for a short time (less than an hour) and for a task, for which they lacked ownership; also, including more participants would have given more statistical power for comparing conditions.
%
Future work should perform experiments with more realistic and longer-term summarization engagements. 
%
Regarding our datasets, we chose two to differentiate between formal writing (i.e., news articles) and informal writing (i.e., social media posts).
%
However, we did not experiment with more societally critical summarization tasks, such as medical or legal documents. %\joel{I have two major problems with this sentence:  1. if they aren't important then why did we select them?  2.  They actually can be important.  For example, a lot of people don;t have time to read long news articles and just want the tl;dr.  Especially the case when there are muleiple articles on the same story.  Social media (tl;dr) may seem silly, however, there are definitely applications for summarizing a whole comment thread (to understand arguments etc) for example, which the Reddit dataset can be seen as a first step towards}
%
While post-editing was useful when more domain context was needed, it is unclear how our findings would generalize to more high-risk scenarios.


% \alison{I don't think this belongs in the limitations; perhaps in future work but would need a bit of editing}
% Another aspect that was not explored in this work is the idea of skill transferability in text summarization.
% For example, how long does it take for someone who is trained on summarizing financial articles to post-edit a AI-generated medical article?
% Since advanced models can be easily built to generate summaries for new datasets, there is a possibility for humans to pick up summarizing skills on unfamilar domains in a shorter duration of time.
% However, since the time taken to train a person manually and by AI-assisted text summarization systems are unknown, future work can explore the benefits and drawbacks of skill transferability on unfamiliar domains in text summarization.

% \para{Post-editing in text summarization is useful for unfamiliar domains.}
% %Manual summarization is typically high quality but time consuming, whereas automated summarization is more efficient but with reduced quality; therefore, we want to understand how pairing human and AI affects efficiency and quality.
% %Ideally, we want post-edit to improve quality compared to automatic summarization and (either) improve quality or efficiency compared to manual summarization. 
% %
% %
% Comparing post-editing to manual summarization, the results were mixed. 
% This mixed effect 
% % is well documented in literature on post-editing in machine translation 
% is observed in some post-editing machine translation studies \cite{koponen2016machine}. 
% They show that while post-edited machine translation can reach a similar quality as manual translation \cite{Plitt2010APT, garcia2010machine}, others find that manual translation is more preferable in terms of style \cite{fiederer2009quality}.  
% %
% While \datareddit does not show promising results, 
% % (manual outperforms post-edit for quality), 
% % likely because of especially poor quality provided references, 
% for \dataxsum, allowing post-editing leads to similar summary quality as manual with improved efficiency, suggesting that assistance is more helpful in unfamiliar contexts, i.e., 
% % \dataxsum is a dataset of British-related articles and 
% the majority of our participants are not familiar with
% % were more familiar with Reddit than with 
% British-related events and news. 
% %
% We also found support for this speculation from machine translation literature, which shows that despite the lack of domain knowledge about the language, monolingual editors can perform high quality translation tasks with the support of machine-generated translation \cite{koehn2010enabling}.  

% % Echoing prior literature on post-editing in machine translation~\cite{green2013efficacy}, post-editing improved the quality in both the \datareddit and \dataxsum experiments compared to automatic summarization. %post-editing allowed users to improve the quality of the provided summary. 
% %
% % While this is not surprising, it further exemplifies such a need for human intervention when high summary quality is desired.

% \para{Users need better starting points for post-editing.}
% The low quality of the assistance provided for post-editing in Reddit may have limited participants in those conditions:\joel{not sure what the participants has  to do with the situation} manually summarizing outperformed post-editing in quality and efficiency. 
% %
% This is contradictory to existing literature about post-editing in machine translation, where post-editing can generally boost human efficiency~\cite{Plitt2010APT, flournoy2009machine}. 
% %
% % This surprising result may be due to the fact that Reddit self-summarization in the form of TL;DRs is not always coherent or accurate; 
% % \ke{the regression analysis tell different story that less coherent provided summary lead to better post-edit summary compared to manual summary} \viv{right, this is actually correct. mmm how should we explain this}; 
% % for example, post authors sometimes use this medium to make a joke or summarize in incoherent lists.
% %
% % Therefore, using these summaries as references can be problematic.
% %
% %
% % Another possible explanation is the possibility of over-reliance on low quality summaries. 
% %
% %

% As described in our results, some participants were not sure what to edit as the provided summary seemed good enough for them while others deferred to the provided summaries instead of spending time understanding the important points and summarizing themselves. 
% %
% It is possible that these participants over relied on provided summaries and could not discern the areas that need improvement. 
% Previous studies on text generation have indicated that users may consider provided summaries as an ``authority'' and thus feel apprehensive to make significant edits~\cite{bhat2021people}. 
% %
% The lack of the background knowledge about specific domains might also exacerbate this issue.
% %This was demonstrated by manual summarization outperforming post-editing in quality and efficiency.

% % \para{On the need for better reference datasets.}
% % \alison{this subsection needs a little work, (1) let's talk more generally about the importance of good reference datasets and what our results tell us (that existing reference datasets aren't great); (2) it could be a call to action for the community (whether to explore new ways of extracting human references or collecting them more efficiently); (3) include related work that evaluates reddit, xsum and other summarization datasets; Joel linked to some I believe (e.g., Maynez et al. 2020)?} \viv{Maynez et al. 2020 evaluated halucinated content in AI-generated summaries but i don't think it's related to the original dataset itself. it's more of the model problem} \ke{This seems to be a bit off from the main topic of the paper. More relevant would be given that we know some dataset have low quality in their provided reference summary, our study indicate that AI-Human collaboration help build high-quality summary dataset. But we should start with expert written summary (manual summary has the highest quality), train the AI model, use AI model as assistance to guide and transfer the knowledge for non-expert to summarize better and more efficiently}\alison{let's shorten this and discuss two points: (1) that current reference datasets are low quality which can be problematic and (2) that approaches like ours can be used to improve references (although asking people to manually summarize also could work based on our results..)}
% % \alison{in an earlier section we talk about reddit references being bad and that affecting performance in that condition, but here, let's talk more generally about the importance of high-quality provided summaries and why we need better reference datasets}
% For both \datareddit and \dataxsum, the provided summaries (AI-generated and human reference) were lower quality than those produced by humans in our study.
% %
% Existing literature suggests that it is often more efficient for human users to post-edit human-generated text than machine-generated text, as text produced by human is often higher quality. 
% %
% For example, it is faster for physicians to edit medical consultation notes generated by other physicians compared to notes generated by AI models~\cite{moramarco2021preliminary}. 
% %
% The same pattern has also been observed in machine translation, where human-translated text needs smaller amount of edits and time spent than machine-generated translations~\cite{zouhar2021neural}.
% % \joel{the last few sentences feel like a rehash of what was said in the first part of the paper to motivate this work}
% %
% Given that incoherent references hindered the summarization process,\joel{correction: hindered some of the post-editing.  Also many of them weren't incoherent, they just weren't a canonical summary (which I am assuming is what is desired here)} it is important to have high-quality references summaries.\joel{have to be careful - if they were high quality, then we don't need post-editing.  Another way to put it is that the summaries should be of some threshold of quality?  }
% %
% High-quality reference datasets also serve as a jumping-off point for models to generate better summaries.\joel{this sentence seems out of place}
% %\alison{this point is interesting because it shows how fine tuning a LM can actually overcome some reference issues (reddit model generated were better quality than the reference) whereas typically the algorithm goal is to reproduce the reference; not sure whether/how to discuss that, though}
% %For \dataxsum, the references were rated better than the AI-generated summaries, but for \datareddit, the references were worse than the AI-generated summaries.

% % References serve as ground truth and might assist humans to summarize better.
% % \alison{too many ``mights'' in this paragraph, what does our data tell us?}
% % Since \datareddit references were of poor quality, participants might have felt frustrated and abandoned the provided summary and wrote a new summary instead of using the provided one.
% %Since the \datareddit references were of poor quality, some of the participants commented that ``It might have been easier to do "blind" summaries rather than having the provided examples''. (\datareddit, \condhuman)
% %If participants had to summarize a more formal writing text (e.g., doctors' notes), they may have less trust towards the provided summary or the system when constantly shown poor quality summaries.

% % \viv{tried addressing the challenge ``deciding what was important from the original document'' in the last sentence. i'm not sure what related work should be discussed here}
% % We used \dataxsum for formal writing and \datareddit for informal writing but both datasets have their downsides.
% % Many participants commented that it was 
% % difficult to summarize \dataxsum news due to lack of domain knowledge and 
% % confusing to summarize \datareddit posts due to incoherence of the provided summaries.
% % Additionally, the content of some \datareddit posts can be a long ramble without any main points, making the summarization task more difficult than it should.
% %
% % As such, the community should either explore new ways of extracting human references or use humans to create new and better quality reference datasets.
% \joel{one has to be careful here because this paragraph undercuts the whole experiment.  If the underlying was wrong to begin with, then what can we learn?}

 


% %\subsection{Design Recommendations}
% % \alison{tutorials and instructions can probably be combined into a recommendation (and is more specific to the study design than on the actual system}
% %\para{Systems should support tutorials and give clear instructions.}
% \subsection{Design Recommendations for AI-assisted Text Summarization Systems}
% % \alison{need to shorten this and perhaps break out into specific recommendations (what are they?)}
% %\alison{beyond tutorials and better instructions, can we suggest what qualities to strive for in AI assistance for summarization based on qual and quant results (what did people like or not like about the provided summaries? when was manual better?) perhaps we suggest that AI assistance only be provided in some cases..? any other ideas like that?}
% %\alison{until we add other specific design reccs, I folded the tutorial recc into the main discussion}
% % Our findings shed light on the design of future AI systems to assist human users in text summarization. 

% \para{Consider user interactions with AI assistance.}
% % We found that not all participants appreciated provided summaries as reference for their own writing. 
% % Some were confused about incorrect information presented in the reference summary, some thought the summary disruptive and would rather write independently, others showed tendency of over reliance on the AI-generated summary and do not feel confidence to add their own edits. 
% Our qualitative results suggest that there are various factors that could influence post-editing quality. 
% % On one hand, we as 
% While NLP researchers should work on improving the quality of AI-generated summaries or suggestions so they can be helpful references in human summary tasks,
% % On the other hand, we as developer of human-AI systems 
% we should also consider extending how user interact with AI assistance. 
% For example, users could benefit from a design that they have the ability to turn off AI assistance when they do not need it to reduce distraction. 
% A workflow design where human users first write their summary independently before getting AI assistance might help with the issue of over reliance. 
% Features that allow users to raise questions and issues about AI-generated summaries in a community with other human users and AI developers could also help users more effective work with AI summaries.    

% \para{Provide tools to combat uncertainty.}
% % Another strand of user challenges came from working with the original text. 
% % Some participants commented that they do not have enough background knowledge about the domain presented in the article so it is hard for them to fully comprehend the original text. 
% % Others found that it was challenging to  figure out what information was important to be included in a summary or was confused about the expectation on the summary. 
% The design of future system should consider addressing the following user needs: (1) insufficient background knowledge about the domain; (2) lost about relevant information that should be included in a summary and confused about the expectation on the summary.
% First, systems could provide users with effective background and contextual information. 
% For example, users can benefit from inline web-searching or dictionary features embedded in the original text that they can use to learn more about the domain. 
% Second, users could benefit from scaffolds in the original text that hinted important information. 
% % Perhaps in addition to generating a summary for the user to post-edit on, 
% AI assistance could also take in the form of highlighting key points in the original text. 
% Lastly, systems should provide users with proper training and effective tutorials to set expectation on the quality, style, and format of the summary. 
% For example, a checklist could be implemented so user could know whether their summary meets the criteria; tutorials in text summarization interfaces can also take in the form of interactive recap or mini test to ensure users are clear on what to do in the task.
% A handful of participants also commented that they found it difficult to summarize due to poor delivery of the original articles.
% Although the main problem stems from the original documents, 
%Properly trained users and comprehensive tutorials in text summarization interface could help with the process.
% \para{Provide clear instructions.}
%Despite the tutorial and practice provided, participants were unsure what to expect in writing a good summary.
%The current interface might not be clear, thus text summarization interfaces should list clear instructions on what to expect from the users.
%This was one the most frustrating issues in the study.

% Of course, all these design suggestions are merely speculations based on the insights from our study. We call for future research effort to develop novel AI-assisted summarization systems and rigorously investigate design choices through user studies and experiments.
%\para{Support additional features.}
% \alison{this is a good idea but we need to back it up.. do we have any comments from participants asking for additional supports?}
%\viv{regina, could you help look for comments that support this? i believe there was at least one that mentioned some other features.}
%Additional features could be included to assist user in the process.
%For instance, highlighting phrases, leaving comments and making notes on the original document.
%Since the current interface provides only the original text and a text box for the summary, it could be further improved to emulate the process of students taking lecture notes.


% \subsection{Limitations}
% One limitation of our experiment is that we are unable to control all potential confounding factors that could possibly impact our results.
% In our experiment, we controlled the reading speed by ensuring that the participants in the same condition had similar reading speed.
% However, there are other factors that are not within our control.
% For future work, before deploying a human-centered AI-assisted text summarization system, it is advisable to first perform a large-scale A/B testing experiment in production environment.
% Additionally, our results do not generalize and might not be applicable for other datasets.
% This is especially true \ke{human post-edit does not help for Reddit does not mean it is not a good results. If we use another dataset also with bad reference, we might get similar results. I think our finding is indeed generalized on the point that ``Users need better starting points for post-editing.''} with regards to \datareddit as the references provided in the original datasets are not well-written, unlike other well curated datasets such as \dataxsum.


%While the results have given insights on how post-editing affect summary quality, efficiency, and user experience, it also shows what could have been done in retrospect.
%Many of the participants who are exposed to the \dataxsum dataset commented that the summarization task was difficult due to lack of domain knowledge.
%This is mainly attributed to the fact that many of our participants are from the United States while the \dataxsum articles are based on British culture and news.
%Although we did a check on the participants' knowledge on British culture, for future references, it would have been more insightful to use a dataset that the majority of the participants understands.
%For instance, while a handful of the participants felt that it was difficult to understand the \datareddit posts, none of the participants expressed that they find the summarization task difficult due to lack of domain knowledge.

% We chose two datasets to differentiate between formal writing (i.e., news articles) and informal writing (i.e., social media posts), and we anticipated the references provided by those datasets to be ``high-quality'' provided summaries for post-editing. 
%
%However, the low coherence of the \datareddit reference summaries might have affected the results and limited the value of assistance 
% \ke{bad reference is not the limitation of the study. From our study, we get to know what could be a better AI assistance in the case of post-editing, i.e., better quality of provided summary, no matter it is from human reference or AI-generated.}. 
% \viv{we need to change this. according to regression analysis bad coherence actually leads to better post-edit summary compared to manual summary}
%
% However, both datasets had lower quality human reference summaries compared to the summaries produced in our experiments, which likely limited the value of assistance.
%
% Further, many 
% Participants were less knowledgeable about British news in \dataxsum and summarizing \datareddittifu posts is not a particularly realistic or important summarization task, compared to summarizing medical or legal documents, for example.
% %
% While post-editing was useful when more domain context was needed, it is unclear how our findings would generalize to more high-risk scenarios.
% %
% Future work should consider better quality references and more realistic summarization datasets.
%Turkers rated reference summaries as lower quality than model-generated summaries, suggesting that providing reference summaries might be more of a hindrance than of a help.
%On the other hand, it is worth noting that one of the differences between informal and formal datasets might be the quality of the reference summaries.
%Overall, using informal datasets such \datareddit acts as a double-edged sword and might influence the results and insights to a certain extent.

% Even for highly trained annotators, human evaluations of generated text are subject to variability.
% %
% Although we took care---through pay rates, tutorials, attention checks, and validation---to ensure that crowdworkers understood how summaries should be rated and worked hard during the task, they may still be rushed or unsure of how to rate, which might result in ratings that would not match experts.
%
%While we removed outliers when cleaning the data, some documents might be affected as we collected only five samples from each document.
%
%For instance, if a turker is disqualified due to failed attention checks, and that some of remaining turkers' responses are outliers, that document will have less samples as compared to other documents.
%Additionally, since there is no ground truth to compare annotator' ratings, calculating true agreement rate \ke{did we check the agreement rate, or correlation of ratings between annotators} is not possible.
%
%We attempted to maintain the integrity of quality ratings by disqualifying ``bad'' annotators in every batch deployed (see Appendix).
%
% Therefore, our results are limited by the quality of our evaluation, and it remains open to discussion on how the community can effectively gather higher quality human labels.

==> Vivian 2021 Dataminr Internship Project/sections/intro.tex <==
%!TEX root = main.tex

\section{Introduction}
\label{sec:intro}
%\alison{important to remember we're writing to the *CL audience for the human-centered nlp special theme, so let's describe how prior focus in text summarization has been on algorithm improvements and automatic evaluations, and while some use humans for evaluation, far less work has actually brought human into the summarization process (cite those that do); therefore, this work aims to explore how human and machine can work together for summarization, specifically whether providing assistance in the form of editable summaries improves humans summarization quality, efficiency, and experience compared to human or machine alone.}
Text summaries provide short overviews of long documents or document collections, allowing readers to understand the content without the need to read full documents.
%
For example, news summaries outline key points so that readers do not have to read the entire article.   
%
For scientific papers, abstracts allow readers to easily understand the extent of the work and decide whether the paper is relevant to them.  
%
%Summaries are traditionally written by humans with domain expertise: journalists write summaries for news articles while researchers write abstracts for scientific papers.
%
% \alison{is there a slightly different description and cite we could use here? otherwise this looks a bit too similar to regina's paper} \viv{updated}
While these human-written summaries are typically high quality, a human's time and energy is limited and such tasks require heavy cognitive load~\citep{kirkland1991maximizing}.
% ~\cite{hidi1986producing}.
%
%Skills are also not transferrable, and specialized domains are best summarized by humans with expertise (i.e., medical notes, legal memos).%\joel{too complicated...reduce double negative?}

Therefore, increasing research effort has explored machine models to generate summaries automatically~\cite{tas2007survey,nenkova2012survey, ELKASSAS2021113679}.
%
%Advanced models can be trained on large corpora of ``reference'' summaries and finetuned to other datasets (for which there are adequate references),
% \joel{note that not all summarization algorithms operate using fine-tuning} 
% in theory,
%solving the problem of skill transferability that a human might face~\cite{liu-lapata-2019-text, lewis2020bart}.
%
While recent advances in learning algorithms and data have resulted in models that can generate relatively high-quality summaries, human summarization is still the gold standard.
%
Further, training models require large, high-quality summarization datasets that are expensive to curate.

%In recent years, human-AI collaboration has risen as a promising paradigm for tasks that include AI models and humans as important components of the process to work together towards achieving a goal.
%Given the pros and cons of human and AI summarization
Taking advantage of the complementary strengths of humans and AI, can they \textit{collaborate} to improve summarization performance? 
%for better text summarization---whether to produce training datasets or for downstream summarization tasks?
%
%Since post-editing has been successful in other text generation tasks (machine translation), where post-editing 
In the area of machine translation, a common method of human-AI collaboration is human post-editing of AI-generated text, which increases human productivity and improves the quality of translation~\citep{koponen2016machine,vieira2019post}. 
%
However, in spite of its potential impact, studies of post-editing for summarization have been very limited, e.g. \citet{moramarco2021preliminary}, in the medical domain.
%

%\alex{In spite of its importance, and potential impact, studies in Human-AI collaboration in summarization tasks, however, have been very limited. NOTE: are we 100 percent sure moramarco is the ONLY work that addresses this? (e.g. \citet{moramarco2021preliminary}, in the medical domain. In this paper, we present... } \alison{general human-ai collab for summarization is limited, and especially so for the specific technique of post-editing: moramarco is the only work Viv found on it}
%
%Inspired by this, \citet{moramarco2021preliminary} explored post-editing in text summarization, suggesting it could potentially increase human efficiency. 
%
%However this study was conducted on small scale with only a handful of participants. %,lending credibility to the hypothesis that post-editing could help to improve text summarization.
%Thus there lacks a formal understanding of whether post-editing can help humans in summarization tasks.%, let alone how we can effectively incorporate post-editing in future summarization systems. 
%
%In fact, \citet{moramarco2021preliminary} recently showed that post-editing improved efficiency for summarization, but on a small scale (3 participants).
%, suggesting potential in post-editing for summarization tasks.

%\alex{the inspired by this paragraph seems out of place here}
To bridge this gap, we performed a large-scale human subject experiment  (72 participants) investigating the utility of post-editing provided summaries in text summarization for informal (Reddit) and formal (news) datasets.
%for summary quality, efficiency, and user experience.
%
We expect tradeoffs in quality and efficiency (i.e., it might take longer to write better summaries), so we are interested in whether post-editing can actually improve efficiency or quality over manual methods, as well as the effects on users' experience.
%
This work is an important step 
%\joel{first...or second? given the Moramarco '21 cite }\alison{the first to do it at larger scale - moramarco was 3 people}
toward understanding the benefits and drawbacks of post-editing as opposed to manual text summarization.
%We conducted a large-scale human subject experiment to find out whether post-editing can improve efficiency or quality over manual through the three measures: summary quality, efficiency, and user experience.

%\alison{findings/takeaways need to be updated (build from what is in the abstract)}
%Our results are mixed %but are within the expectations of tradeoffs between quality and efficiency (e.g., it might take longer to write better summaries).
% Participants improved on AI alone: 

%\joel{something to consider - this paragraph starting: post-editing yielded better.... do we need it?  we don't necessarily have to say what happened completely up front.  Food for thought if we are low on space } \alison{sure we can drop the findings summary if needed for space}
%Post-editing yielded better quality summaries than the automatic methods. 
% %
%However, compared to manual summarization, the results were mixed.
% 
%For news, post-editing lead to similar quality summaries with improved efficiency.
%
%However, post-editing produced worse summaries, more slowly for Reddit.
%
%From open-ended responses, post-editing was most useful when participants lacked domain knowledge but was problematic when the provided summaries were inaccurate. 
%
%Further, participants had different editing strategies (i.e., some made many changes---regardless of provided summary quality---while others made fewer), suggesting the need for custom solutions based on participants' preferences and domain. 
%Our findings suggest that humans have different goals of summarization that are not always evident and post-editing allows humans to tailor a summary to their goals or a particular audience, prompting future work in exploring effectiveness of post-editing in text summarization.
%

Our main contributions can be summarized as follows:
%\alex{needs a little work}: \joel{need to make sure that the sentence structures are parallel in the enumeration (I tried to fix it up) }
(1) we present the first large, human subjects experiment of post-editing for text summarization; (2) we show how post-editing impacts summary quality, efficiency, and user experience---where it is useful and where it is not; and (3) we create, and make public, two new datasets, each with 360 human-evaluated summaries for news and Reddit posts---either written manually or post-edited on provided summaries.%\joel{make sure to emphasize the data release}


%\joel{maybe it is cleaner to say "recent advances in learning algorithms and data have produced models which can generate...."  something like that?  "Due to advances in technology" is vague.  }
% has allowed researchers to create better models that lead to improved performance in text summarization and other downstream NLP tasks.
% To evaluate how well a model performs on the text summarization task, new measures such as ROUGE \citep{lin2004rouge} and BLEU \citep{papineni2002bleu} are proposed by researchers.
% With correct resources and architecture, 
% Models can easily train a model 

%
% Yet, while models generate summaries more quickly than humans, human performance is still the gold standard.
% Prior work has also shown that ROUGE score does not correlate well with human evaluation \citep{liu2009exploring}.

% Since both humans and models have their pros and cons, the idea of human-AI collaboration emerged in recent years. 
%Human-AI collaboration allows models to assist humans in identifying counterintuitive patterns in data and humans help make up models' inability to make rational decisions. 
%Prior work has experimented human-AI collaboration in domains such as sentiment analysis \citep{hase2020evaluating,nguyen2018comparing}, (visual) question answering \citep{feng2018can,chandrasekaran2018explanations}, and topic modeling \citep{smith2018closing}.
%\alison{I'm not sure how the following few sentences relate to our paper; instead, maybe just a quick sentence on the importance of understanding how users want to interact with AI systems and their experience when doing so?}f
%Human-centered systems empower and assist humans to perform the task better.
%While the majority of the tasks do not directly impact a human, there are some tasks decision that concern ethical and legal reasons requiring a human to make the final decisions (e.g., recidivism prediction, medical diagnosis), making studies in human-AI collaborations and human-centered systems meaningful and impactful for societal needs.

% human vs. machine summaries
% \alison{should we go into extractive vs. abstractive in the intro or save for related work?}
% There are two methods in generating summaries, extractive and abstractive.
% The extractive method creates the summary by extracting important sentences from the original document while the abstractive method creates the summary by identifying important messages, interpreting and reproducing the summary in the shortest way possible.
% To generate high quality summaries, supervised methods with high quality ground truth data are often recommended.
% Since current methods have yet to surpass human written summaries, they are regarded as the gold-standard for ground truth labels.
% While human labeling ensures high quality summaries, it is costly and not scalable.
% On the other hand, although generated summaries are not as high quality as human written summaries, they are scalable and less costly.
% \alison{let's find other interactive nlp cites to use that don't break anonymity}
% To capitalize the advantages of both models and humans, human-AI collaborations are becoming more popular and widely used in different sub fields in NLP such as machine translation [] and topic modeling \citep{smith2018closing} to improve quality of the final product (e.g., translation,).
% Recent text summarization research has largely focused on algorithm improvements and automatic evaluations \cite{WIDYASSARI2020, Gehrmann2021TheGB}.%\joel{do you mean recent summariation research?}
% %
% % \alison{fill in cites}
% While humans are frequently used for annotation or evaluation \cite{bhandari-etal-2020-evaluating}, it is less common that they are brought into the text summarization process. 
% %
% And, prior work has not yet explored human-AI text summarization at a large scale. 
% %
% Yet, human-AI collaboration is a promising paradigm, shown to both improve human and model performance in other NLP domains, such as sentiment analysis~\citep{hase2020evaluating,nguyen2018comparing}, question answering~\citep{feng2018can,chandrasekaran2018explanations}, and topic modeling~\citep{smith2018closing}.\joel{I think you have to be very clear  about why it is promising since we don't know what reviewers one will get.  Do those citations show work where humans helped the AI or vice versa?  Are there examples of this research really providing a benefit.  Then the justification to pursue this path is stronger.}

% \joel{I think it is important to lay out scenarios where one would do }
%
% Therefore, we explore how humans and machines can work together for text summarization, specifically whether providing assistance in the form of editable summaries improves human summarization quality, efficiency, and experience compared to human or machine alone.
% %
% %We explore how pairing human and AI affects efficiency, quality, and user experience for text summarization with 
% In a between-subjects experiment, 72 participants write summaries with or without AI assistance for formal (news) and informal (Reddit) datasets.%\joel{I feel this might have been two sentences?}
% %Note that AI-assistance and post-editing are used interchangeably throughout the paper.
% % We employ 72 participants to write 720 summaries and hire another 113 participants to evaluate 1440 summaries.

% For the human-AI pair to be successful, post-editing would improve quality over automatic methods and either improve quality or efficiency compared to humans summarizing manually.
% Unsurprisingly, humans improve on AI alone: post-editing outperforms automatic methods. 
% %
% However, compared to manual summarization, i.e., without AI assistance, the results are mixed.
% %
% For news, post-editing lead to similar quality summaries with improved efficiency.
% However, post-editing produced worse summaries, more slowly for Reddit.
% %
% %Further analysis and 
% Participant's open-ended responses suggest low quality Reddit reference summaries are to blame.
% %Post-editing improves summary quality as compared to the quality of provided summaries.
% %Additionally, providing summary as a form of assistance improves the final summary quality to a certain extent as compared to when assistance is not provided.

% This work contributes: 
% (1) the first large, human subjects experiment of AI assistance (post-editing) for text summarization; (2) understanding how AI assistance impacts summary quality, efficiency, and user experience---where it is useful and where it is not; and (3) two new datasets, each with 360 human-evaluated summaries for news or Reddit posts---either written manually or post-editing provided summaries.

% \joel{my initial thoughts on the introduction are that it can probably be shortened.  Skip to what your hypothesis more quickly and lay out why this is an important research question and what you hope to see.  I think this can be done with 2-3 fewer paragraphs.}


%for XSum and Reddit-TIFU datasets; \ke{more specific on conditions. Not sure we should tell the dataset name here. Say them earlier in the intro.}
% (4) introduces a novel 
% \ke{expect more details on the novel parts in following sections?} \viv{there is a paragraph titled `eliminating the bad apples' in section 4 which is dedicated to the novel method. should it be elaborated more?} \alison{let's discuss with Joel whether to include this method as a contribution (I do think we did something interesting but is it a ``novel contribution''?)} 
% method \viv{to be confirmed with joel} to collect human labeling data from crowdsourcing platforms 
%and (4) recommend design guidelines for human-AI text summarization systems. 
% \alison{another contribution might be design guidelines for future systems?} 
% \viv{is this a new section in discussion?}

% \alison{we can probably cut this structure piece; the motivation, summary, and contributions in the intro are much more important IMO}
% The paper is organized as follows: (1) Related work where we cover prior work contributions and our inspiration; (2) Summary collection where we describe the first of the two steps in collecting human written summaries; (3) Summary evaluation where we describe how we executed the process of evaluating summaries collected from the previous phase; (4) Results and insights answer the overarching research question if provided assistance improves summary quality, efficiency, and user experience; and lastly (5) Discussion and conclusion of this paper.

==> Vivian 2021 Dataminr Internship Project/sections/method.tex <==
\section{Evaluating Post-Editing for Text Summarization}
\label{sec:method}
%\joel{I think this section needs to start higher level.  Explain the experimental flow, the control, etc.} 
We explored
% \joel{we need to make sure tense is consistent across the paper} 
how providing summaries for post-editing affects (RQ1) final summary quality, (RQ2) efficiency, and (RQ3) user experience, compared to fully manual or fully automatic approaches for two domains: social media and news. %\joel{we should either cite the datasets here (note they are in 3.1, OR we just say the domains are social media and news}
%
Participants reviewed documents and summarized them, either without any assistance (manual) or provided with a human-written or AI-generated summary that they could edit (post-edit).
%
A distinct set of annotators then evaluated the quality of the summaries.
%
%\alison{is this a fair assumption? it didn't turn out.. should we back off and say we just expected human references to be better?}
We included both human-written and AI-generated summaries in our study to explore post-editing for different summary types and qualities. %, as we expected that human summaries would be higher quality than those generated by AI. %\ke{Note for Joel: we use the wording of ``post-editing of AI-generated text'' a lot, but we also have ``post-editing of human reference summary'', to make the ``AI-generated'' more generalized, can we say reference summary can be considered as generated from an oracle AI model}.\joel{Ke: I'm not sure what you mean. Can the AI system really be an oracle in this case? It's imperfect}
%\alex{maybe i missed it, but we talk about summaries and references and its unclear if they're the same thing? i see that below it's clear what the difference is. terminology should be consistent and clear in the order it appears, so this section should clarify- IF we use those two terms, what they mean..}\alison{let's not talk about references until we get into the data}
\subsection{Data and Model}
We chose social media posts and news articles for our study as they could be understood by a general audience and are commonly experimented with automatic summarization literature. %: Reddit posts and news articles.\joel{this is repetitive with the above.  Especially since above XSUm is mentioned but here it isn't.}
%
We also chose these datasets as they vary in writing formality, which might impact how humans understand and summarize text. 
%
Specifically, we used the \datareddittifu dataset~\citep{kim2018abstractive} (informal, Reddit ``Today I F'd Up'' posts) and the Extreme Summarization (\dataxsum) dataset~\citep{narayan2018don} (formal, British news articles). 
% \joel{there should be examples of these datasets or at least the references somewhere} 
%
Each of these datasets includes  human-written ``reference'' summaries for the original documents: \datareddittifu uses the ``TL;DR'' written by the author of the post\footnote{Reddit users often self-summarize their posts with ``TL;DR:'' or ``too long; didn't read:'' statements.} while \dataxsum uses the introductory sentences---written by journalists---as the summaries (see \tabref{tb:example_summaries}).
%\joel{need to be consistent in the ordering of the datasets.  So far it has seemed Reddit goes before XSUM but in this paragraph it gets flipped around.  Need to keep it that way all times.}
% \alison{refer reader to the document/summary examples in the appendix}

For participants to summarize during our study,
we randomly selected 120 documents from the test sets (10 documents per participant, per condition),\footnote{\href{https://huggingface.co/datasets/reddit_tifu}{Reddit-TIFU}, \href{https://huggingface.co/datasets/xsum}{Xsum}} with length between the 25th and 75th percentile to balance task difficulty and time.
% \alex{as a reader, i'd be curious to know the lenght distribution of the collections- if its in the original paper, good to cite here}\alison{viv can you handle?}
The average length of the \datareddit posts is 243.8 words, and the average length of the \dataxsum articles is 223.3 words (see Appendix \ref{app:doc_len_dist} for length distribution).

We used the Pegasus model~\cite{zhang2020pegasus} to generate summaries for the two datasets. 
% \alex{important to explain why we used pegasus and not a different one. later in the paper, important to explain any tradeoffs or limitations of having used this one vs anotehr one}
% \alison{viv or ke can you handle?}
% \viv{this is implicitly answered in the last few sentences of this para: it achieves SOTA and it has readily tuned models available}
% \ke{Yea, the model is first pre-trained using masked language model, then fine-tuned on each specific dataset, but not by us. Ke will add more here}
Pegasus is a masked language model pre-trained with a novel self-supervised objective, gap-sentences generation, and fine-tuned on downstream abstractive summarization tasks. 
%\alison{can we take off the human-level performance piece OR explicitly describe what is meant by that.. either way it contradicts us: (1) we said earlier that the ai generated isn't as good as the reference: (2) in intro, we say that ai generated is not as good as human}
The model achieved state-of-the-art performance on multiple datasets, including \dataxsum and \datareddittifu. 
% \joel{make sure to say that we are using the default settings (if we are).  Btw, was the model tuned for each of the datasets?  So are we using a Pegasus model for Reddit and one for trained for XSUM?  Or just a generic model?  }
% \alison{viv or ke can you handle?}
% We used the finetuned models with default configuration that are available on Huggingface for each dataset.
We directly applied the off-the-shelf Pegasus models downloaded from HuggingFace, with one already finetuned on \dataxsum \footnote{\href{https://huggingface.co/google/pegasus-xsum}{huggingface-pegasus-xsum}} and the other on \datareddittifu \footnote{\href{https://huggingface.co/google/pegasus-reddit_tifu}{huggingface-pegasus-reddit\_tifu}}.
% \viv{ke does this sound right?}
% \viv{We did not use weaker summarization models as the goal of the paper is to understand if humans are able to write better quality summaries when given good quality summaries generated by models as assistance.}
% \alison{

We did not introduce summaries from any other models besides Pegasus, as the goal of this paper was not to compare models but to understand how human post-editing of provided summaries compares to manual and automatic methods. 
%
And, while Pegasus is currently high-performing compared to other, weaker models, the summaries we provided for post-editing in our study were of varied quality, particularly between datasets (see \secref{sec:results:quality}).
This gave us an opportunity to explore how summary (or assistance) quality might affect human post-editing.
% }  

% The base Pegasus model was trained with stochastically sample important sentences and we use the fine tuned models for the respective datasets 
% \ke{the performance of the model does not tell much. we just say the model is one of SOTA models for both datasets}
% The models used are one of the SOTA models for both datasets.
% (\tabref{tb:pegasus_performance}).

%Finally, we built a simple web application to facilitate the experiment. 
%and conducted a pilot study before running the full user study.
%Read appendix for more details of the pilot study.
% \footnote{The web application went through a few rounds of iteration to ensure that the wordings and flow was correct and easy to follow.We did two pilot study sessions, the first was conducted among researchers with 5 users mainly to get feedback on the usability of the web application and the average duration of a session, and the second one was conducted with actual targeted users on Upwork.} 

\subsection{Study Design}%\alex{this secton needs a sentence clarifying that there were 2 phases: (1) writing of summaries, and (2) evaluation of the summaries. then, in the sub-sections below, it should be clear. for example, the participants section doesn't explain that it applies only to phase 1 (the mturkers are, effectively also participants). this creates a lot of confusion for the reader. it think fixing that will address some of my comments below}
This study consists of two phases: (1) summary collection and (2) human evaluation of the collected summaries.
% \alison{we should probably explain why we used two different types of provided summaries (AI generated and references) and what we expected} 
%\condgen references are more scalable while \condref are more expensive.
%As such, we are interested to find out the differences in effects of the types of provided summary as assistance.
For summary collection, we used a between-subjects experimental design, with three conditions: (1) \condmanual, where participants wrote summaries without any assistance; (2) \condai, where participants post-edited AI-generated summaries; and (3) \condhuman, where participants post-edited human-written summaries.
%
Participants summarized either informal \datareddit posts or formal \dataxsum news articles.
%where participants wrote summaries either: without assistance (\condmanual) or provided with summaries they could post-edit: AI-generated summaries (\condai) or human-written summaries (\condhuman). \joel{the commas and colons in this paragraph make interpreting this paragraph challenging.  Can we just use bulletpoints or something to make it clear what the name of the condition is with its description?}\alex{agree. same thing happens earlier in the paper. a more common, and better style is something like: we used three condtions: (1), .. (2), .. (3)..}
%
For the \condhuman condition, participants were provided the human written ``reference'' summaries from each of the datasets. %\alex{terminology: above we use reference, here we're calling it reference summary..}
%
%
In the following, we describe the participants and procedure for the summary collection phase, followed by details of the evaluation phase.
%We experimented with post-editing text summarization for informal \datareddit posts and formal \dataxsum news articles.


\begin{table}[h!]
    \small
    \centering
    \begin{tabular}{p{0.1\textwidth}p{0.15\textwidth}p{0.15\textwidth}}
    \toprule
    % \multicolumn{2}{c}{Reddit & Xsum} \\
     & Condition & WPM (M, $\sigma$)\\ \midrule
    \datareddit & Manual & 334, 113 \\
     & AI post-edit & 374, 175 \\
     & Human post-edit & 363, 104 \\ \midrule
    \dataxsum & Manual & 327, 112 \\
     & AI post-edit & 360, 241 \\
     & Human post-edit & 396, 178 \\
    \bottomrule
    \end{tabular}
    \caption{Average reading speed per condition per dataset. WPM represents words per minute. 
    % \alison{Viv, can you confirm they are not significantly different? if they are not, write something like, ``Strategic assignment to conditions ensured no significant differences between reading speed.''}
    Strategic assignment to conditions ensured no significant differences between reading speed.
    }
    \label{tb:reading_speed}
\end{table}

\subsection{Summary Collection Participants}
% \alex{was country part of the selection criteria?}\alison{viv can you handle?}
We recruited 72 participants (45 female, 22 male, 3 non-binary, 2 preferred not to disclose) from  Upwork.\footnote{https://www.upwork.com; we used Upwork---as opposed to other crowdsourcing platforms---to recruit experienced participants and ensure higher quality summaries.}
%
They were on average 32 years old ($\sigma$=12) and were required to be native or bilingual English speakers, have at least a 90\% job success score, and possess expertise in writing, journalism, or communication.
%The country of residence was not part of the selection criteria.
%
To ensure participants had some familiarity with the summarization domains, they described their experience reading or posting on Reddit and knowledge of British news.
Specifically, participants rated the extent of the respective knowledge based on a 7-point Likert scale, and were selected if they responded at a rating of 4 or above.
%
Finally, participants reported their reading (in words per minute, WPM) and comprehension scores,\footnote{https://swiftread.com} which we used to (1) eliminate those with comprehension less than 75\% and (2) account for reading speed when assigning conditions.
%\viv{moved paragraph below from appendix}
To account for differences in participants' reading speed that could affect our results, we assigned participants into conditions, ensuring a similar average reading speed across conditions (\tabref{tb:reading_speed}).
%
%The metric used is words per minute, as represented by WPM.
%
The average reading speed for participants in our study was 358 WPM ($\sigma=158$). 
% \ke{are each pair significantly different or not?}


\subsection{Summary Collection Procedure}
\label{sec:procedure}
Based on pilot studies (see Appendix \ref{app:pilot}), we anticipated the summary collection task sessions would take an hour and we paid participants \$20.
%
Each participant took on average 33.9 minutes ($\sigma$=15.0) to perform the summarization task.\footnote{Participants spent additional time completing the post-task survey.}
%
Of the 72 participants, an equal number (12) were randomly assigned to each dataset (\datareddit or \dataxsum) and summarization condition (\condmanual, \condhuman, \condai), ensuring a similar average reading time for each condition (see \tabref{tb:reading_speed}).
During the study, participants completed three phases: (1) instructions, tutorial and practice, (2) summarization task, and (3) post-task survey.

% \alison{can we move this sentence on research experiment ethics to the appendix?}
% By agreeing to work on the task, participants knew that the summaries collected were for a research experiment. 
Participants first reviewed task instructions, the criteria for writing a good summary (from \citet{stiennon2020learning}), and examples of good and bad summaries with explanations. 
%
For consistency, we used the same criteria when asking annotators (a distinct set of human evaluators) to evaluate the summary quality. %(see \secref{sec:human-eval}).
%
%\alex{this sentence is unclear. did participants know if the source was manual or ai generated? it's also unclear, in general, IF a participant summarizes a document or a collection of documents- a reddit post is never defined above.. }
Participants then reviewed 10 documents (either all \datareddit posts or all \dataxsum news articles, depending on their assignment) and summarized each, either manually (\condmanual) or post-editing a provided human summary (\condhuman) or AI-generated summary (\condai).
%
\figref{fig:upwork_task_interface} shows an example of the task interface for the \condai condition and \dataxsum.
%
Participants were not made aware of the source of their provided summaries--whether human or AI.
%
%\alex{terminology.. to a participant summarizes a summary or a document?? if its a reddit it's neither..? very confusing}
Per condition, each participant summarized a unique set of 10 documents.
%
Participants had access to the summarization criteria as guidance while summarizing.
%
After completing each summary, participants rated the difficulty for summarizing the original document.
%
Finally, after finishing all 10 summaries, participants completed a survey about their experience.
See \ref{app:phase1_procedure} for details on the procedure and tutorial examples.
%  and task interface.

\begin{figure}[t!]
    \centering
    \begin{subfigure}[t]{0.5\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figs/upwork-task-interface.png}
    \end{subfigure}
    \caption{Sample task interface for the \condai condition for \dataxsum, showing the provided, AI-generated summary in the text box.}
    \label{fig:upwork_task_interface}
\end{figure}


\subsection{Human Evaluation of Summary Quality}
\label{sec:human-eval}
%While we can measure summary quality using automatic measures (ROUGE), such measures do not typically align well with human quality ratings~\cite{liu2009exploring}.
%
To evaluate the quality of the summaries written during our study, we recruited a distinct set of annotators from Amazon Mechanical Turk.
%\viv{Due to scalability issues, we employed annotators from Amazon Mechanical Turk instead of Upwork. }
%
To ensure quality ratings, we only employed turkers who satisfied the following criteria: (1) completed 5000 HITs; (2) 97\% HIT approval rate; (3) reside in the United States, Australia, and United Kingdom.
% \alison{again, can we move this line about ratings being collected for research to the appendix?}
% By agreeing to work on the HITs, turkers knew that the ratings collected were for a research experiment. 
 %and were allowed to perform multiple HITs, as we assume they would improve at the evaluation task over time.
% \joel{can someone calculate how much per hour they would make?  That is a point people discuss these days now.  I just want to have the number ready and maybe include it in the paper if it is above minimum wage}\alison{i think its in the appendix and its not good (like 6.50 an hour) but we think our average time is inaccurate.. because turkers are sneaky and take multiple HITs then complete them in parallel. We only track time from when they accept to complete the HIT}
%
Annotators underwent tutorials and multiple attention-check questions before performing the task (see \ref{app:evaluate_summary}).
%
We also eliminated annotators with validation procedures (see \ref{app:quality_control}).
%
Annotators were paid \$1.50 per HIT (see \ref{app:evaluate_summary}) and were allowed to perform multiple HITs, assuming they would improve at the evaluation task over time. 
% \alison{@viv - can you report on how many average HITs annotators did?}
Each annotator performed 9.4 HITs on average.


The annotators evaluated six different summaries for each original document (\dataxsum article or \datareddit post) from our study: 
(1) the \condmanual summary written without any assistance,
(2) the summary written in the \condai condition, given (3) the \textit{AI-generated} summary from the Pegasus model, %\joel{it would make it more coherent if all the summary types were clustered.  The way it is set up now is that a summary type is dependent on another summary type.  Might be easier to order things like: 1. Original human reference  2. manual human summary 3. AI generated summary 4. human post-edit 5. AI post-edit, 6. random.  But maybe there is a reason why you went with the original order....it is setting up what the results look like?}\alison{i did this confusing way to save space and try to clarify which summaries were provided in each condition (maybe not important though)}
(4) the summary written in the \condhuman condition,
given (5) the \textit{human reference} from the dataset,
and, finally, (6) a \textit{random} summary generated by randomly selecting two sentences from the opposite dataset.
%
See Table \ref{tb:example_summaries} in \ref{app:example_summary_type} for examples of each summary type.
%
The random summary was used as selection criteria to identify annotators who were not paying attention during the task. %\joel{a note on the word "eliminate"  - obviously this makes sense - we apply a set of filters to whittle down the candidate annotators to ensure we have high quality ones.  I wonder if we can take a positive spin and frame things as "selection criteria"}
% \alison{we need to talk about the different axes they evalute on here and cite stiennon}
% Annotators scored summary quality on four axes: Coherence, Accuracy, Coverage, and Overall on a scale from 1 to 7, following \citet{stiennon2020learning}. 
% \ke{Didn't see definition of the four axes in Appendix. Add a figure there}
Following \citet{stiennon2020learning}, annotators evaluated each summary on four axes: \textit{coherence}, \textit{accuracy}, \textit{coverage}, and \textit{overall}. 
Each summary was evaluated by five annotators; we removed outliers then averaged the remaining annotators ratings to determine the final rating for each summary.
%
%See Appendix for the variance for each condition per dataset.
%
Refer to \ref{app:eval} for additional details on the human summary evaluation procedure, annotators, and quality control.

% \joel{I am ommenting as I read, but what was the rationale for using AMT and not expert human evaluation?  Does this make the results questionable?  Is there prior work that used AMT and found it to be reliable?  That would allay concerns.} \viv{we decided to use AMT for scalability reasons. employing people on upwork would not be feasible}

\subsection{Measures}
\label{para:measures}
We report on {\it summary quality}, {\it efficiency}, {\it user experience} for the summarization task. 
%
Summary quality is measured using human ratings and 
%on four axes (Coherence, Accuracy, Coverage, and Overall), following \citet{stiennon2020learning}.
%
efficiency is measured by the amount of time to read and write a summary for each document.
%
We additionally measured user workload as \textit{edit distance} or the difference between the provided summary and the final summary.
% As it is not simple to extract summarization time from reading time (as participants might switch back and forth between reading the original document and writing their summaries), we measure the time taken from when the participant receives the original document to when they submit their summary.
% We account for individual reading time differences by ensuring a similar average reading speed, measured by words per minute (WPM), between participants (M=358, SD=).

We also report on three subjective user experience measures collected using 7 point rating scales (from strongly disagree to strongly agree) either on the task-level (at the end of the task) or instance-level (after each summary): \textit{task difficulty}, ``I found it difficult to summarize the article well.'' (instance-level); %\textit{understanding},  or ``I found it difficult to understand the content of the article'' (instance-level),
\textit{frustration}, or ``performing the summarization tasks was frustrating.'' (task-level); and \textit{assistance utility}, or ``the provided summaries were not useful to me when I was performing the summarization tasks'' (task-level).\footnote{Only participants in the post-editing conditions responded about the utility of the provided summaries.}
%
All task-level measures were paired with follow up ``why did you feel this way'' open-ended questions. 
%
% \alison{do we report on likes, dislikes, and desired improvements in the results? I removed the part on assistance being useful because that is included in the assistance utility response above}
% We also report on other open-ended responses, including what participants \textit{liked} and \textit{did not like} about the task of writing the summaries and any \textit{desired improvements} to make the summarization process easier.
%
% \alison{do we report on WPM and comprehension? I think this is not a measure for our study, so let's remove}
% Lastly, we report on participants' reading speed measured by words per minute (WPM) and test score on comprehension quiz (comprehension).

\subsection{Data and Analysis}
72 participants wrote 720 summaries (manually or post-editing provided summaries) and 113 annotators evaluated those summaries, resulting in 6360 summary quality ratings; after removing outliers (see \ref{app:quality_control}). 
%
Averaging resulted in one final quality rating (on four axes) for each summary.
%
% \alison{IMPORTANT - viv, we need to provide this data}
We make this dataset of summaries and their ratings public to promote future research.\footnote{https://github.com/vivlai/post-editing-effectiveness-summarization}

To find out if any statistical differences exist between the means of the conditions, we used one-way ANOVA for each objective and subjective (rating scale) measure.
%
Using post-hoc Tukey's HSD, we also performed pairwise comparison to determine which two conditions are significantly different.
% For significant main effects of \textit{AI Assistance}, we used post-hoc Tukey's HSD.\joel{most NLP people will not know what that sentence means}   
%We report on all significant results, including pairwise comparisons. 
%

We qualitatively coded the open-ended responses related to the subjective measures of frustration, task difficulty, and assistance utility, as well as responses on likes, dislikes, and desired improvements.
% A researcher in the team first manually coded the data and iteratively developed themes from answers of each question. 
% For example, "lack of context knowledge" is one of the themes developed from the answers to the question about why participants rate the task as difficult. 
% The researcher then discussed the themes with the team, merged and updated the themes, then re-coded the data again. 
% To validate the coding results, a second researcher also coded the data based on the themes developed by the first researcher. 
%\alison{can you report the exact kappa score? also give details on how you both rated - was it a set subset of all responses? or some number from each open ended question?}
%\viv{kappa score is stated below and we elaborated more on thematic coding in appendix. added a sentence below to ask reader to refer to appendix}
One researcher read the data to identify emergent codes, followed by a discussion period to merge and update the themes in the codebook. 
%
Two researchers then independently coded all the open-ended responses respectively, achieving a high average inter-rater reliability (Cohen’s $\kappa >= .85$) for each of the open-ended responses.
%
See \ref{app:thematic_coding} for details on thematic coding.
%
We refer to participants as P1-P72.
% 1-P72. %(dataset, condition). 


==> Vivian 2021 Dataminr Internship Project/sections/related.tex <==
%!TEX root = main.tex

\section{Related work}
\label{sec:related}
%\alison{let's cover more about automatic summarization and lack of human collab (discuss how humans primarily used for providing training data or evaluating except in limited circumstances.. there are some examples of human collab during summarizations right? need to include all them and explain their limitations (since we claim to be the first large study)}

\subsection{Automatic Text Summarization}
The field of automatic text summarization can be traced back to 1950s \citep{luhn1958automatic};
% \joel{you need to have cites from the 1950s, not links to the survery papers} 
and since then much research has been devoted to developing algorithms, datasets, and evaluation metrics to developing summarization systems that can approach the quality of a human ~\cite{ELKASSAS2021113679}.
% \joel{note my rewrite}
%
There are two primary automatic methods: (1) \textit{extractive}~\citep{dorr2003hedge,Nallapati2017SummaRuNNerAR}, where the model selects important sentences from the input document, and (2) \textit{abstractive}~\citep{rush2015neural,paulus2017deep}, where important parts of the input document are paraphrased to form new sentences.
%
While recent deep learning-based summarization methods have significantly advanced the quality of AI-generated summaries, they face some common issues, including hallucination, also known as contextual inconsistency~\citep{maynez2020faithfulness} and factual inconsistency~\citep{cao2018faithful,kryscinski2019evaluating}.
%
% \alison{for the human labor part, do we have cites? do we mean post editing or something else?}
These critical issues limit the utility of automatic summarization if unaddressed; in fact, 
% human labor is often employed to manually fix these mistakes for important summaries
humans can be in the loop to manually fix identified mistakes, thus iteratively improving AI models~\citep{zhang2012active, gidiotis2021uncertainty}.

\subsection{Human Text Summarization}
Summaries written by humans often serve as gold standard references to train and evaluate AI models \cite{bhandari-etal-2020-evaluating}. One natural source of human summaries is shared and collected on the web, e.g., titles of news articles \cite{DBLP:conf/acl/SeeLM17, narayan2018don}, TL;DR of Reddit posts \cite{volske2017tl,kim2018abstractive}, talk transcripts of scientific papers \cite{lev-etal-2019-talksumm}, and government bill summaries \cite{kornilova-eidelman-2019-billsum}. 
Those are generated to serve specific goals and audiences, and often contribute datasets at scale to build AI models, although the data quality is not guaranteed
% \joel{what is meant by large-scale here?} 
% One drawback is that these summaries 
% \joel{need to define noisy here} 
~\cite{kryscinski-etal-2019-neural,bommasani-cardie-2020-intrinsic}. 
Alternatively, human summaries can be annotated by dedicated professionals or crowd-workers for domain-specific documents \cite{jiang-etal-2018-effective}.
% Before automatic methods were developed, summaries were traditionally summarized by humans.
% Human-written summaries serve a couple of purposes: (1) annotated data that acts as a gold standard to train more accurate AI models~\citep{} and (2) for downstream tasks~\citep{} \viv{need to explain this}.
% Human summarization are performed by one human~\citep{} or human to human collaboration~\citep{}.
Annotators are often trained with guidance and summarization criteria, yet quality control~\citep{daniel2018quality}, due to subjectivity and inconsistency between annotators~\citep{tang2021investigating}, is a challenge. 
While the annotation process is costly and time-consuming,
% \joel{is the issue inefficiency or just that it takes a long time?  I think the latter.  Why not say "time-consuming" insread}, 
% \joel{expert or otherwise?} 
human summarization, often by domain experts, yields higher quality compared to automatic methods \cite{zhang2020pegasus}. 
% \viv{added the point on experts given joel's comment}
In this work, we turn to a common method of human-AI collaboration---human post-editing of AI-generated text---as an exploration for a viable solution.
% When employing a distinct set of annotators to perform the summarization task, 
% While annotators are trained and given guidance during some summarization tasks, this process is highly inefficient and costly.
% As compared to automatic methods, human summarization often yields higher quality but need well-trained humans or domain experts, which can rack up cost very quickly~\citep{??}.
% With both pros and cons of automatic and human methods for text summarization, 
% we turn to a common method of human-AI collaboration---human post-editing AI-generated text---as an exploration for a viable long-term solution.


% \alison{per Ke: discuss related work of humans producing summaries (for training data, for downstream task, maybe human-human post editing?; and issues of using human summaries for model training}
% \alison{this needs a good bit of updating; I'm skipping for now}
% To produce accurate results for supervised models, labelled data is often crowdsourced on platforms.
% As such, annotation has a long history since the beginning of supervised machine learning.
% While the process has been around for a long time, the human summary annotation process is still filled with challenges and issues.
% Common issues include factual inconsistency between annotators~\citep{tang2021investigating} and quality control~\citep{daniel2018quality}.
% One of the main challenges faced is that one reference is treated as the gold standard but does not fulfill the criteria of different goals and audience~\citep{}.
% \citet{} discuss the issues in current existing summarization datasets.


\subsection{Post-Editing AI-Generated Text}
%The field of human-AI collaboration has shown promising results in the text generation process~\citep{wang2021putting}.
%Similar to text summarization tasks, text generation systems incorporate human evaluation as the final step to ensure quality~\cite{khashabi2021genie}. 
%For example, \citet{clark2018creative} presented a machine-in-the-loop creative writing system where the users provided prompts to the model and the model generated suggestions that users could accept or decline.
% \alison{does this prior work in MT show that post-editing is successful? and if so, for what cases? need to give an example}
Post-editing is a common technique in machine translation, where translators edit the translations produced by automatic methods (opposed to completing the translations manually).
%
% \alison{should we include the viera cite here as well?}
It has been shown to increase productivity and improve translation quality~\cite{Plitt2010APT,koponen2016machine,vieira2019post}, particularly when initial translations are good.  However, post-editing longer segments can require more cognitive effort to identify errors and plan corrections~\cite{koponen2012comparing}.

As summarization shares similarities to machine translation, post-editing is a promising paradigm, yet it is underexplored. 
%While post-editing shows promise for other text generation tasks, yet post-editing for summarization is under explored.
%
% \alison{make sure we relate our findings on edit distance back to this cite} \viv{added}
One exception is \citet{moramarco2021preliminary}, who evaluated post-editing in the medical domain.
In a study with 3 physicians, participants took less time to post-edit other physician's written notes as compared to AI-generated notes, and post-editing any type of notes was faster than writing an entire note from scratch.
% \joel{I added "an entire note from scratch"}
%
Participants' 
% \joel{the authors or the doctors?} 
note-taking style differences also affected post-editing time.
%
For example, Doctor A wrote shorter notes and only edited AI-generated notes when there were substantial issues while Doctor B was more meticulous and edited the AI-generated notes extensively.
%
We build on prior work and explore post-editing for text summarization at a larger scale (72 participants) over two domains.
% \alison{I don't think our goal was to investigate on less specific domains.. it was to investigate at larger scale whether post editing is effective}
%To investigate how post-editing affects text summarization on a larger scale, we present the first large-scale human subject experiment to date (72 participants) to formalize understanding of AI assistance in text summarization from the human perspective.

% \alison{talk more broadly about human-AI collab for summarization (or maybe even text generation); about autocomplete and other methods before going into post editing. Include more papers with specific details from the lit review spreadsheet}
% As summaries generated by AI alone are often low quality~\cite{huang2021factual, durrett2016learning}, many view AI as an assistant instead of replacement of human work \cite{dellermann2021future}. \joel{it's weird to say summaries are of low quality when, in the intro, it is claimed that "models can generate relatively high-quality summaries".  } 
% %
% Humans can \textit{collaborate} with AI in text summarization and, more generally, text generation tasks, in different ways.
% %
% Humans can make edits and check for grammar and spelling on auto-generated text (often referred as ``post-editing'')~\cite{green2013efficacy}; many text generation systems also incorporate human evaluation as the final step to ensure quality~\cite{khashabi2021genie}. 
% %
% Emerging research has also explored novel ways for humans to actively control the text generation process~\cite{wang2021putting}. For example, \citet{stiennon2020learning} integrated human feedback in the model training process; \citet{clark2018creative} presented a machine-in-the-loop creative writing system where the users provided prompts to the model and the model generated suggestions that users could accept or decline; \citet{passali2021towards} offered an interactive visualization tool that allowed users to view and control self-attention weights and other hyper parameters in text summarization models.

% Despite this prior work, it remains unclear if and how human-AI collaboration actually improves the \textit{human} summarization process. \joel{one should go into the prior work for human-AI summarization in more detail.  Most people don't know these citations} 
% %
% %\alison{how does our work relate to green? do we find similar results? different?}
% For example, there are mixed signals about whether post-editing yields higher quality text~\cite{koponen2016machine}. 
% %
% Similarly, AI assistance can boost human productivity \cite{Plitt2010APT}, yet editing AI-generated content can also take high technical and cognitive effort \cite{koponen2012comparing}. 
% %
% These uncertainties suggest a lack of formalized understanding of AI assistance in text summarization from the human perspective. 
% %
% Furthermore, most prior research efforts examining AI assistance in text summarization involved localized, small scale (n<=10) user studies (e.g., \cite{akoury-etal-2020-storium, moramarco2021preliminary}), providing only initial understanding. 
% %
% To bridge this gap, we present a large-scale human subject experiment  (72 participants) to investigate the effect of AI assistance (post-editing) in text summarization for summary quality, efficiency, and user experience.  \joel{this sentence right here is the best summary of the goals of the paper so far} 

%, using post-editing as an example of human-AI collaboration. 
%
%We build on prior work in this study, which offers the first known large scale investigation of human-AI collaboration for text summarization with 72 participants. 
%There are different types of AI assistance in text generation, autocomplete and post editing.
%Autocomplete is mainly used in creative writing such as slogans and stories writing \citep{clark2018creative}.
%Post editing is commonly used in machine translation where human annotators edit the generated translations as models are still far from perfect as compared to translators.

%In this paper, we investigate how post editing affects the text summarization.

% The idea of post-edit came from machine translation.
% Since the translation generated models are not perfect but acceptable, human annotators or translators edit the generated translations.
% Given that the premise is similar, we incorporated post-editing to our text summarization task.
% The idea of post-edit overlaps with a popular interdisciplinary topic in computer science, human-AI collaboration.
% In a human-AI collaboration, humans are complement to the AI.
% While models are more accurate and are able to identify counterintuitive patterns in datasets that humans are unable to see [], there are things that the AI is unable to accomplish simply because it is not a human.
% Additionally, due to many reasons, especially ethically and legally, humans should be the gatekeepers when making the final decision to a task.
% Although text summarization does not directly affect a human's life nor associate to any type of risks, the motivation of having access to AI assistance is to assist humans to perform the task of text summarization better.
% In the ideal scenario, with AI assistance, humans are able to summarize better quality summaries in the same amount of time or shorter time.

% which creates an abstract representation of the input text and produces summary texts with words or phrases that might not appear in the original document. 
% Recent deep learning-based summarization methods have significantly advanced the performance of AI-generated summaries. %They are often supervised models learnt to generate golden-standard human written summaries.
% Popular neural \textit{extractive} methods often formulate and solve summarization as a classification problem, where the encoder learns sentence representation and the classifer scores their importance of being part of the summary~\citep{Nallapati2017SummaRuNNerAR}. 
% SummaRuNNer \cite{Nallapati2017SummaRuNNerAR} is one of the earliest neural approaches adopting an encoder based on Recurrent Neural Networks. 
% State-of-the-art models, e.g., MatchSum \cite{zhong-etal-2020-extractive} and BertSumExt \cite{liu-lapata-2019-text}, leveraged pre-trained language model based on Transformers to learn better text representation for extractive summarization. 
% On the other hand, neural \textit{abstractive} methods formulate summarization as sequence-to-sequence problem and learn an encoder-decode architecture to generate summaries in an auto-regressive manner~\cite{rush-etal-2015-neural, nallapati-etal-2016-abstractive}. 
% Finetuning pre-trained large-scale language models on downstream summarization tasks, e.g., BertSumAbs \cite{liu-lapata-2019-text}, T5 \cite{raffel2020exploring}, BART \cite{lewis2020bart}, and Pegasus \cite{zhang2020pegasus}, achieves state-of-the-art summarization performance across datasets. %We use Pegasus for our experiments. 
% domains
% Automatic text summarization systems have been introduced for various text domains, including news, articles, online reviews, legal documents, meeting notes, social media posts~\cite{ELKASSAS2021113679}.
% % \joel{each one of the different domains would ideally have a cite}  
% We focus on a formal (news from \dataxsum dataset) and an informal (social media posts from \datareddittifu) source text domain as our case study. 
% We use the off-the-shelf pre-trained Pegasus model, which reports state-of-the-art performance for the two datasets~\cite{zhang2020pegasus}. \joel{seems early to be introducing which model we are using} 
% evaluation 
% AI-generated summaries are automatically evaluated by comparing with human-written ``reference'' summaries, often measured by the ROUGE score; ROUGE-N measures the number of overlapping ``n-grams'' between the model-generated summary and reference~\citep{lin2004rouge}. As ROUGE does not correlate well with human judgements~\cite{liu2009exploring}, human evaluation is commonly used~\cite{bhandari-etal-2020-evaluating}; as such, we use human evaluation for our experiments.
% The closer the ROUGE score is to 1, the better the generated summary.
% However, recent prior work has also shown that the ROUGE score is not a comprehensive measure and should only be taken with a grain of salt \citep{liu2008correlation,liu2009exploring}.

==> Vivian 2021 Dataminr Internship Project/sections/results.tex <==
\section{Results}
\label{sec:results}
We report on the impact of post-editing on summary quality, efficiency, and user experience.

\subsection{Summary Quality}
\label{sec:results:quality}
%
% We used human evaluation to compare differences in the quality of the produced summaries during the summarization task.\joel{I say we remove this sentence (above).  We already know this from the last section.} 
%
We discuss quality ratings for the summaries for each dataset (\figref{fig:quality_overall_coherence}).
%
For simplicity, we report only on \textit{overall} quality ratings from the human evaluation (see Appendix~\ref{app:acc_cov_ratings} for other axes).
% \joel{this subsection needs some structure.  Maybe lead off by saying we will discuss each dataset and that a summary of the results are in Figure 1?}
%
% Automatic methods exist but do not typically align with human judgements~\cite{liu2009exploring}. 
%
% To confirm, we compared human evaluation ratings to ROUGE-1 (Spearman correlatio), finding no strong relationship ($p=.11, \rho=-.07$ for \datareddit, $p<.01, \rho=-.3$ for \dataxsum).
% \joel{I think you should commit to using human evaluation and leave it at that; assuming you feel confident with the human eval.  If you're going to say you looked at the correlation, probably a good idea to actually state the correlation numbers}  
%The overall and coherence rating are used to compare correlation to ROUGE-1 using Spearman correlation.
%In \datareddit, we find weak significant correlation for overall ($p<.01$) ratings to ROUGE-1.
%For \dataxsum, we find weak significant correlation for coherence ($p<.01$) ratings to ROUGE-1.


%when comparing differences.
% Overall quality 
%which is the primary metric for comparing differences between the 
% generated summaries. 
% and coherence plays an important role in provided summary utility (as we will show by regression analysis and open-ended responses).
% the results hold for the other axes (coherence, accuracy, and coverage; 
%We additionally explore correlations between human and automatic evaluation, edit distance 

\begin{figure}[t]
    \centering
    \begin{subfigure}[t]{0.5\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figs/reddit-xsum_overall.pdf}
        % \caption{Overall rating.}
        % \label{fig:quality_overall_combined}
    \end{subfigure}
    % \begin{subfigure}[t]{0.5\textwidth}
    %     \centering
    %     \includegraphics[width=\textwidth]{figs/reddit-xsum_coherence.pdf}
    %     \caption{Coherence rating.}
    %     \label{fig:quality_coherence_combined}
    % \end{subfigure}
    \caption{Average \textit{overall} quality ratings 
    % (overall and coherence) 
    for the summaries by type and dataset. For \datareddit, the human reference was the worst (aside from the Random summary). For \dataxsum, the AI-generated summary was the worst.}
    \label{fig:quality_overall_coherence}
\end{figure}

\para{For \datareddit, post-editing improved the quality of the provided summaries but manual summaries were the best.}
% primary reddit quality findings
\datareddit summaries produced by participants in the \condmanual condition %($M=5.8, \sigma=0.9$) 
were rated highest \textit{overall} quality; the provided summaries, \condgen %($M=4.7, \sigma=1.0$) 
followed by the \condref %($M=4.4, \sigma=1.0$) 
were the lowest quality (\figref{fig:quality_overall_coherence}).
%
Interestingly, our evaluation finds that the AI-generated summaries are significantly higher quality than the human references ($p=.02$). This is different from \citet{zhang2020pegasus},
% \alison{viv add the pegasus cite?}, 
for which the same Pegasus model achieved comparable performance to human references (but not better).
%\joel{In prior work that used Reddit, was the machine better than the original human reference?  That is what Fig 1 is showing.} \ke{The paper of the model we used actually achieve human-level performance, they did a human eval and ratings are the same as human reference although no significant winner} \alison{question for Joel: should we explain this? it is not too surprising that the machine is better because ai-generated is less likely to pull in extra details and is more coherent (since its fine tuned from pre-trained summarization model) overcoming issues with the reddit references}
%\joel{I think it is always good to say if we are seeing similar patterns as the prior work or different patterns when repeating an experiment.}
%\viv{ok so should we cite the work and say that we got differnt results?}

Comparing summarization conditions, we find significant differences for final summary quality ($p<.01, F=9.3$): \condmanual summaries outperformed summaries produced by participants in both the \condai ($p=.03$) and \condhuman ($p<.01$) conditions.
%\joel{these two ideas don't seem to go together.  I read this as 1. AI assistance improves summary quality.   2. Manual is better than post-edit.  Each should be its own sentence, unless I am missing something here.} \alison{its confusing because we first report on the anova results (whether there is a difference in any conditions, then report on pairwise which tells us which conditions were significantly different} 
%
%However, the quality of the final summaries for the post-edit conditions did not differ significantly ($p=.13$).
%
Finally, summaries resulting from \condai and \condhuman were significantly better than the provided summaries for those conditions, \condref ($p<.01$) and \condgen ($p<.01$), meaning participants improved the quality of the summaries they were given.
%


\para{For \dataxsum, post-editing improved the quality of the provided summaries and was just as good as manual.}
% primary xsum quality findings
\dataxsum summaries produced by participants in the \condmanual condition were rated the highest and the provided summaries (\condref followed by \condgen) were the lowest (\figref{fig:quality_overall_coherence}).
However, for \dataxsum, summary quality was not significantly impacted by \textit{AI assistance} ($p=.08, F=2.5$), meaning there was no significant difference in quality between the \condmanual, \condai, or \condhuman summaries.
% \joel{what is the explanation?  I guess we could measure how extensive the edits were}\alison{no real explanation but this is a good result - that participants summaries were just as good when they wrote manually as when post-editing} 

%Exploring whether participants improved on the provided summaries for \dataxsum, pairwise comparisons with correction again showed that 
Similar to \datareddit, \condai and \condhuman summaries were significantly better than the provided summaries for those conditions ($p<.01$). %, \condgen ($p<.01$) and \condref ($p<.01$), respectively. 
%
But, opposite of \datareddit, the \dataxsum \condref summaries were significantly better than the \condgen summaries ($p=.02$).

%\viv{should we still have this paragraph but talk about open ended responses instead? we actually covered a bit of that (assistance utility open-ended responses) in user experience section. also, title should probably not by provided summary coherence}
%\alison{no, we need to remove this and instead discuss open ended responses in user experience}
%\para{Provided summary coherence impacts post-edited summary quality}
% To explore when post-editing is most useful and not useful 
% valuable (i.e., when post-editing outperforms manual summarization quality), 
% % we used regression analysis (see \figref{fig:quality_regression_analysis} in Appendix) to determine which features of the task and the participants impacted whether a post-edited summary was higher quality than the manual summary (for the same document).
% we conducted thematic coding and analyzed qualitatively using open-ended responses.

% For \datareddit, provided summary overall ($p<.01$) and coherence ($p<.01$) ratings, participant reading comprehension score ($p<.01$), and perceived task ease (i.e., reported summarization difficulty) ($p=.01$) had a positive impact on whether the post-edited summary was rated better quality than the manual summary; for \dataxsum, provided summary coherence ($p<.01$), reading comprehension score ($p=.03$), and document length ($p<.01$) had positive impact.
% %
% For both datasets, the coherence of the provided summary was important for how well participants performed when provided with that form of assistance.


%Comparing between datasets, the coherence ratings were significantly higher for \dataxsum provided summaries (\condref and \condgen) than for \datareddit ($p<.01$).
%
%In fact, \datareddit human references were the lowest scored (for Coherence) of any of the summary types we evaluated (except for the ``Random'' summary).
%
%Therefore, the low quality of the assistance provided for post-editing in \datareddit may have limited participants in those conditions (see \secref{sec:discussion}). 

\subsection{Efficiency}

\para{Post-editing human references slowed \datareddit summarization but post-editing AI-generated summaries was faster for \dataxsum.}
Summarization conditions significantly differed in efficiency (\figref{fig:efficiency_comparison}) for both \datareddit ($p=.04, F=3.2$) and \dataxsum ($p=.02, F=3.8$).
%summarization condition significantly impacted efficiency ($p=.04, F=3.2$, \figref{fig:efficiency_comparison}): 
For \datareddit, it took significantly longer to post-edit human references (\condhuman) than manually (\condmanual, $p=.03$) or given AI-generated summaries (\condai, $p=.02$). We discuss possible reasons for this (e.g., problematic Reddit references) in \secref{sec:reddit-difficulty}.
%\alison{come back to this to ensure we add a quote and refer back about inaccurate reddit references to the latter section; otherwise update here with different redit quality}
%. but no significant difference in efficiency between the \condmanual and the \condai conditions ($p=.90$).
%For \dataxsum, \textit{AI assistance} significantly impacted efficiency ($p=.02, F=3.8$, \figref{fig:efficiency_comparison}). 

% \alison{reporting numbers without mathmode saves space but looks bad -- what is typical for ACL?}
For \dataxsum, post-editing AI-generated summaries (\condai) was faster than \condmanual ($p=.11$) or given human references (\condhuman, $p=.08$).
% \joel{I think there is an obvious story for why Reddit ones took longer.  }\alison{what is it? that reddit references are hard to understand and therefore take a long time to review and update?}
% \ke{p-value seems not right, given the bar chart with confidence bar here} \viv{i double checked it is correct. to be exact it's 0.0768 when comparing human post-edit and ai post-edit}.
%
However, no pairwise comparisons were significant after correction.\footnote{Based on the trend, we would expect to see a significant result with more statistical power (more participants).}

\begin{figure}[t]
    \centering
    \begin{subfigure}[t]{0.5\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figs/reddit-xsum_time_taken_in_minutes.pdf}
    \end{subfigure}
    \centering
    \caption{Comparison between conditions for average time to summarize (per document) for \datareddit and \dataxsum. In general, participants in \dataxsum took longer to complete the task, likely due to unfamiliarity with the domain.
    % to time taken to read longer news articles 
    %\ke{do we have numbers to support this?}\alison{do you mean the average length of xsum vs. reddit documents? agreed that would be good to mention somewhere}\ke{Yes to Alison's question} \viv{average reddit article has more words than xsum. added that information to method section in data. changed the reason to unfamiliarity with domain knowledge}. 
    % \ke{the y axis name is wrong!}
    }
    \label{fig:efficiency_comparison}
\end{figure}

\para{Provided summary quality did not impact the number of edits.}
%does the quality of the assistance (provided summary) affects how much work the humans need to do}?
%To determine whether provided summary quality impacts workload (or how many edits the human must make during post-editing), 
Anticipating that participants might have needed to make more edits to improve on worse summaries, we compared the edit distance to provided summary quality (overall) using Spearman correlation.
%\alison{I'm not sure if we report this as a weak correlation or none? does .2 count as a correlation?}
%\viv{i think it's still very weak} \alison{its too weak to report}
However, for neither \datareddit nor \dataxsum, did summary quality have a strong relationship to edit distance.
%, we find a weak significant correlation for overall ($\rho=0.2, p=.02$) and coherence ($\rho=0.2, p<.01$) ratings to edit distance.
%For \dataxsum, we find no significant correlation for provided summary quality to edit distance.
% \alison{we should provide a little more explanation and detail here as this finding could impact design guidelines for future systems: (1)it would be good to see the chart for this (at least in appendix); I think it's all over the place (in some cases people made many edits to good and bad summaries, in other cases they made very few edits to good and bad summaries), need to describe that in the text; (2) it would be interesting to see if particular participants tended to make more or less edits (meaning some people just feel the need to make changes regardless of how good the summary is); (3) another possible explanation is that in some cases only a few edits are needed to improve a bad summary?}
In some cases participants made many edits to both good and bad summaries, whereas in others, they made very few edits regardless of quality (see \ref{app:edit_distance} for correlation plots), due in part to participants' diverse editing styles, where some desired to make changes regardless of the provided summary quality; \citet{moramarco2021preliminary} made similar observations.
% \joel{it would be cool to make a scatter splot where one axis is the quality and the other axis is the number of edits} \viv{yes we did. included in appendix though, should we move it to the main paper? @alison}\alison{no room, I refer reader to the correlation plots in the appendix}
%
For example, P10 (\datareddit, \condai) ``did not use [the provided summaries] at all'' and P55 (\datareddit, \condhuman) edited all the summaries to match their preferred writing style, stating ``I found the casual writing style confusing [...] I just did it my way.'' 
%
%On the other hand, some participants made fewer edits, instead relying on the provided summaries.
%
%For example, P6 (\dataxsum, \condhuman), ``the provided summaries deterred me from writing my own and gleaning my own major points [...] I would defer to the information given in the provided summaries.''
%
%P31 (\dataxsum, \condai) gave an alternate strategy, ``I learned to read the passage, write my summary, and then look at the given summary otherwise it clouded my memory of what information the passage had actually provided.''
%
%For example, for some participants who were exposed to same dataset and assistance type, and made similar comments about provided summary quality, the edit distance differs.
%\alison{are there any comments about editing strategies? e.g., did any participants say they edited almost all or almost none? or did anyone say they wanted to edit to make it match their style or preference?}
%\alison{comparing these two participants is interesting but would be better if we reported the average provided summary quality they got -- if it is the same, then this is more telling}
%P71 (\datareddit, \condai) whose average edit distance is 240, commented that some of the provided summaries were excellent, and some were awful.
%P52 who has same set up as P71 made similar comments ``only about half were useful'' but had an average edit distance of 138.
%Similar observations are reflected in \dataxsum as well.
%For both datasets, participants made a similar number of edits in an attempt to improve the summary regardless of its initial quality.



% \begin{table}[t]
%     \small
%     \centering
%     \begin{tabular}{p{0.1\textwidth}p{0.15\textwidth}p{0.15\textwidth}}
%     \toprule
%     % \multicolumn{2}{c}{Reddit & Xsum} \\
%      & Reddit & Xsum\\
%     Task ease & $M=2.7$, $\sigma=1.3$ & $M=3.8, \sigma=1.4$ \\
%     Frustration & $M=1.8$, $\sigma=1.2$ & $M=2.7, \sigma=1.5$ \\
%   % Understanding & $M=2.3$, $\sigma=1.7$ & $M=2.7$, $\sigma=1.9$ \\
%     Assistance utility & $M=2.8$, $\sigma=1.5$ & $M=3.0, \sigma=2.1$ \\
%     \bottomrule
%     \end{tabular}
%     \caption{User experience ratings.}
%     \label{tb:user_exp_ratings}
% \end{table}


\begin{figure}[ht!]
    \centering
    \begin{subfigure}[t]{0.5\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figs/reddit-xsum_user_experience.pdf}
    \end{subfigure}
    \centering
    \caption{User experience plots for task difficulty, ``I found it difficult to summarize the article well'', frustration, ``Performing the summarization tasks was frustrating'', and assistance utility, ``The provided summaries were not useful to me when I was performing the summarization tasks'' for \datareddit (Left) and \dataxsum (Right). Responses were collected using 7 point rating scales.}
    \label{fig:user_experience}
\end{figure}


\subsection{User Experience}
\label{sec:user_experience}
% \alison{add chart of user experience ratings and refer to it here}
We measured user experience with \textit{task difficulty}, \textit{frustration}, and \textit{assistance utility} 
% (\tabref{tb:user_exp_ratings}).
% (see Appendix \ref{app:user_experience}).
(\figref{fig:user_experience}).
%In general, participants had more difficulty and were more frustrated, on average, when summarizing \dataxsum than \datareddit.\joel{any reason why this would be the case.  Seems weird that this is the first thing we mention and then move on immediately to another sub topic.  It's also not in bold.} \viv{the first two measures are task difficulty and frustration so we establish that as the first finding. assistance utility is different from the first two measures}\alison{the reason is they lack context for that domain, making it harder (and also, possibly, making post editing better there); but no reason to make this point up front}
%\alison{how does assistance responses compare between datasets? no difference?}
% \alison{instead of reporting all these values for user experience ratings, we could replace with a single chart} \viv{added table. how can we present the table nicely? width of column needs to be bigger but the column is only that big} 
% \alison{what about a bar chart by data type and condition? and under each could we put what the prompt is, something like: task ease: ``I found it difficult to summarize the article well''}
We also surfaced insights about participants' experiences from the qualitative analysis. 

% \joel{other random thought: did you do a coorelation between task difficulty and frustration?  I Would like to think that they would be correlated.} \viv{did some quick analysis here are the results $\rho=.4, p<.01$ for both datasets, see exact numbers below. @alison wdyt}\alison{I think leave off for now unless Joel wants in appendix?}
% (SpearmanrResult(correlation=0.41437144426454714, pvalue=2.274640177613747e-16), reddit
%  SpearmanrResult(correlation=0.42181554239975305, pvalue=5.794252237152267e-17)) xsum

\para{Participants found it harder to post-edit \datareddit references.}
\label{sec:reddit-difficulty}
%but providing summaries did not effect frustration.}
%
%Participants had more difficulty, on average, when summarizing \dataxsum than \datareddit.
%
% \alison{whats a nice (and succinct) way to describe anova results?}
Summarization conditions significantly differed for \textit{task difficulty} for \datareddit ($p=.04, F=3.2$), but not for \dataxsum ($p=.72, F=.3$).
% (\alison{add p and f value}). 
% \ke{we need a definition for ``task ease'', higher score mean more difficult}\alison{yes, agreed: (1) let's switch to ``task difficulty'', (2) we need charts for these measures (task ease, frustration, and assistance utility) instead of reporting all values in text. those charts could include the survey prompts, e.g., ``I found it difficult to summarize the article well''}
Specifically, summarizing when provided a \datareddit human reference (\condhuman) was perceived significantly more difficult than summarizing when provided an AI-generated summary (\condai, $p=.04$).
%
Other pairwise comparisons were not significant.
Recall that post-editing human references also took longer than other conditions for Reddit; this difficultly might be due to the fact that \datareddit human reference data consisted of poorly written TL;DRs, many of which add extra details not found in the original posts. As participants like P63 (\datareddit, \condhuman) and P58 (\datareddit, \condhuman) commented, some provided Reddit summaries were ``really bad'' or ``off a bit.''
%

%Additionally, participants were more frustrated, on average, when summarizing \dataxsum than \datareddit.
%
%Yet, \textit{AI assistance} condition did not have a significant impact on \textit{frustration} for either dataset.

%\para{Providing summaries did not effect frustration or perceived understanding.}
%
%Participants were more frustrated, on average, when summarizing \dataxsum than \datareddit and reported a similar perceived understanding of the original documents for both datasets. 
%
%\textit{AI assistance} condition did not have a significant impact on \textit{frustration} or \textit{understanding} for \datareddit or \dataxsum.
%
%Participants also reported a similar perceived understanding of the original documents when summarizing \dataxsum as summarizing \datareddit posts, and, again, \textit{AI assistance} condition did not have a significant impact on \textit{understanding} for \datareddit or \dataxsum.

\para{Participants were mixed on whether the provided summaries were useful.}
%\alison{this could use another streamlining pass}
\label{sec:results:ux:utility}
%\viv{should we remove mean and variance here? since we already reported it in appendix. mean is in appendix, not variance though}\alison{yes, we should remove mean and variance and move those charts into the main text}
%On average, participants reported low average \textit{assistance utility} for both datasets but with high variability.
%
%Participants in \dataxsum reported that \condref ($M=3.2, \sigma=2.7$) is more useful than \condgen ($M=2.8, \sigma=1.2$) while participants in \datareddit reported that \condgen ($M=3.3, \sigma=1.5$) is more useful as compared to \condref ($M=2.3, \sigma=1.4$). 
%
\textit{Assistance utility} did not significantly differ between summarization condition for \datareddit ($p=.12, F=2.4$) or \dataxsum ($p=.63, F=.2$), due in part to the high variability in participants' responses.
%
However, participants provided mixed responses on the utility of the summaries: while many thought they were helpful ``starting points'' in their summarization process, others found they sometimes missed important points or contained information that was unneeded, incorrect, or incongruous with the original article. 
%

%\alison{do we have some other examples of positive experiences with the summaries? it would be especially useful to include a quote where someone said the summary helped when they needed context.. do we have anything like that??}
Participants, therefore, used the provided summaries in different ways. Some, like P59 (\datareddit, \condhuman) used the summary as a starting point or guideline and made edits on top of it, ``the provided summaries did the job pretty well, I just added some details.''
%
%For example, P35 (\dataxsum, \condhuman) stated that they liked the tasks because they ``have the sample summaries to work off of.'' 
%
%P59 (\datareddit, \condhuman) rated the tasks as not difficult as ``the provided summaries did the job pretty well, I just added some details,'' while  P75 (\dataxsum, \condai), 
Others ignored the provided summary. As P61 (\datareddit, \condhuman) said, ``it might have been easier to do \textit{blind} summaries rather than having the provided examples.'' 
%
Some participants, like P31 (\dataxsum, \condhuman), chose to ``read the passage, write my summary, and then look at the given summary.'' 
%

Participants' had other concerns about post-editing the provided summaries during the task.
%
Some thought it took high cognitive load to make edits and summarize at the same time, ``it clouded my memory of what information the passage had actually provided'' (P31 \dataxsum, \condhuman).  
%
Others struggled with originality. While they perceived it ``a bit like cheating'' (P44 \datareddit, \condai) 
% \viv{note that P44 is actually P81, for record purposes}
% \alison{can we change P75 number too?}
to use the provided summary instead of writing their own, many also ``found it difficult to provide a better summary than what was provided'' (P32 \dataxsum, \condai).
% \viv{note that P32 here is actually P75 in real records}
%
Finally, some participants noticed that they had the tendency to over-rely on the provided summary. For example, P6 (\dataxsum, \condhuman) found that they were distracted from their own thinking and unlikely to challenge the provided summary, ``the provided summaries deterred me from writing my own and gleaning my own major points from the articles. Instead, I would defer to the information given in the provided summaries and edit a few things, but not add anything major.''
% \alison{do we have some more ``not helpful'' examples from Reddit?}
%\para{But, provided summaries could be a hindrance.}
%However, participants also elaborated on the challenges that they faced with the provided summaries in the summarization tasks. 
%
%In many cases, participants felt the provided summary was not helpful. 
%
%For instance, P65 (\dataxsum, \condai) stated that there were some mismatches between the provided summary and the original text, ``some of the prepared summaries made references that were not within the body of text provided.'' 
%
%Faced with incoherent Reddit references, P61 (\datareddit, \condhuman) said ``It might have been easier to do \textit{blind} summaries rather than having the provided examples.''
%
%Both P63 (\datareddit, \condhuman) and P58 (\datareddit, \condhuman) had similar sentiment that some provided Reddit summaries were ``really bad'' or ``off a bit.''
%

%However, comparing assistance usefulness between two types of provided summary in both datasets show different results.


%which corroborates with previous findings that \datareddit references are of lower quality than \dataxsum references.


%
% \alison{since we say ``more'' reddit participants enjoyed the task here, can we be explicit on how many more? especially because above we give 2 xsum examples and 1 reddit}
%Interestingly, 3 more participants mentioned that they enjoyed the task when exposed to the \datareddit dataset, which might be due to the informal, engaging, and comedic nature of \datareddit posts.

%that lack of domain knowledge may significantly handicap the ability to perform the summarization task well.

%\para{Provided summaries were helpful to participants' summarization process but could also be a hindrance.}

% lack of context
\para{Comprehension of the original text can impact summarization.}
%\para{It was challenging to summarize documents that lacked context, were overly detailed, or poor quality.} %and task time constraint challenging.} 
%Results from thematic coding suggest that the disparity of context knowledge about the different original articles might contribute to the different perception of summary quality. 
Participants found it challenging to summarize documents that lacked context, were overly detailed, or had poor quality. 
%
While we intentionally recruited participants with some expertise for the two data types (Reddit posts and British news), many were hindered by a lack of background knowledge, especially for the British news articles (\dataxsum). 
% \joel{have to note that we specifically looked for people with familiarity in these areas...does this mean that the layperson may not be the best source of rater?  } \viv{i think it indicates the down side of self-assessment questions}\alison{yes people are over confident in their expertise - also some of the xsum articles are really wonky}
%
For example, P18 (\dataxsum, \condmanual) said it was difficult to summarize particular articles about ``the British government'' because ``it's not something I am familiar with so it was hard to determine what information to include in the summary.'' 
%
Similarly, P15 (\dataxsum, \condmanual) mentioned difficultly summarizing articles about Cricket, which contained ``sport-specific jargon or proper nouns that I was wholly unfamiliar with.'' 
%A possible interpretation is that, because participants were less familiar with the context of Xsum articles, it is harder for participants to evaluate the quality.
In fact, 50\% of participants summarizing \dataxsum described a \textit{lack of contextual knowledge} compared to only 8\% of participants summarizing \datareddit posts.
%
%\alison{can we write a better version of the following sentence? something more specific?}
Post-editing can help in this case by providing a useful starting point so that users do not need to fully understand the document and write manually.

%
Participants also found it difficult to decide what was important from overly detailed original documents, particularly when summarizing manually. For example, P17 (\dataxsum, \condmanual) stated, ``some articles gave so many details and it took a while to decide which were important to keep in a summary.''
%
Finally, participants were hindered by the poor quality of the original documents. 
%
For example, P60 (\datareddit, \condhuman) viewed the ``lack of capitalization and proper punctuation that is common with Reddit posts'' as the greatest frustration in the summarization process.
%
Participants found it challenging to match the tone and style of these documents in their summaries. 
%
For example, in P46's (\datareddit, \condai) words, it is ``hard to match in the winding, anecdotal writing style often found on Reddit.'' 
% \joel{what guidelines were humans given to summarize?  That obv makes a difference} \viv{we show the tutorial examples and task interface in \ref{app:eval}. a good summary is a summary that satisfies the list of criteria.}
% \alison{describe in discussion how this is another problem with the Reddit dataset and not easy to fix}
%
%


%Finally, time constraint of the summarization tasks seemed to negatively impact the summarization experience. P29 (\dataxsum, \condai) wrote, ``I was a little anxious regarding the time I had left to complete the summaries." %
%P77 (\dataxsum, \condhuman) commented similarly, ``When summarizing I do prefer to make notes as I go on important information, but the time limit had me skipping this to perform the task as quickly as possible."

\subsection{Summary}
Post-editing yielded better quality summaries than the automatic methods. 
% %
However, compared to manual summarization, the results were mixed.
% 
For formal news articles, post-editing lead to similar quality summaries with improved efficiency, helping when participants lacked domain knowledge.
%
However, post-editing produced worse summaries, more slowly for Reddit posts, likely due to the informal writing style and sometimes inaccurate TL;DR references provided in that case.
%
%From open-ended responses, post-editing was most useful when participants lacked domain knowledge but was problematic when the provided summaries were inaccurate. 
%Post-editing improved summary quality over the provided summaries (human reference and AI-generated) for both datasets.
%
%When comparing post-editing to manual summarization, the results were mixed: manually summarizing outperformed post-editing quality for \datareddit, but for \dataxsum, post-editing performed similarly well as manual.
%
%Further, post-editing \datareddit human reference summaries was slower than AI-generated summaries or summarizing manually, whereas post-editing \dataxsum AI-generated summaries was the fastest (compared to manual or post-editing human references).
%
% Regression analysis demonstrated that provided summary coherence \ke{coherence has negative coefficient, thus negatively impact the quality of post-edited summary compared to manual summary}---for which \datareddit references were rated poorly---impacted quality of the post-edited summaries.
%
We did not find a correlation between edit distance and provided summary quality, instead, some participants tended to make more edits---due to style or writing preferences---while others made fewer edits, instead of relying on the provided summaries---regardless of the quality of the summary they were editing. 
%
%
%In general, participants found the provided summaries helpful when they are provided a good starting point for editing, but noted problematic cases where they were incoherent, missing important details, or added extra context that was not in the article. 


% \alison{add a brief summary of the open ended responses}

% \joel{thinking about the summary / conclusions: maybe we should try to generalize a bit more: instead of focusing specifically on the two datasets, speak more generally about formal and informal writing and how that can impact summarization decisions etc}\alison{updated}


==> Vivian 2021 Dataminr Internship Project/sections/study.tex <==
\section{Evaluating AI Assistance for Text Summarization}

We explored how providing summaries (whether from human or AI) for post-editing affects (RQ1) summary quality, (RQ2) efficiency, and (RQ3) user experience, compared to fully manual or fully automatic approaches.
% \joel{this text is very similar to the text in the preceding sentence} 

%To examine the effects of AI assistance and post-editing on the text summarization process, we focus on the following three research questions:
%\begin{enumerate}
%    \item \textbf{RQ1:} How does providing summaries (whether from human or AI) affect \textit{summary quality} compared to manual summarization and automatic summarization?
%    \item \textbf{RQ2:} How does providing summaries (whether from human or AI) affect \textit{efficiency}, as compared to manual summarization?
%    \item \textbf{RQ3:} How does providing summaries (whether from human or AI) affect \textit{user experience} compared to manual summarization?
%\end{enumerate}

\input{sections/method}
%\input{sections/results}

==> sections/data_collection.tex <==
\subsection{Phase I: Summary Collection}
\label{sec:summary_collect}
% \alison{this needs a section or introduction before that describes the full study design and goal and rqs, then you can have a section for details on each phase followed by the results section}
% \alison{let's add in the figs soon to get a better idea on clarity and space}
% \alison{instead of saying what we will discuss in this section, summarize this phase here, something like, ``In this phase, participants review documents (either informal or formal) and provide summaries either without any assistance or post-editing either a model generated summary or a human written reference summary''.}
% In this section, we describe how the first phase was conducted and provide details on the methods and approaches.
% In the first phase of the experiment, 
% Participants first read documents (either informal and formal) then write summaries either without any assistance or provided with a model generated summary or a human-written reference summary.
% We provide details on the study design, protocol, and implementation.

%\para{Methods and Approaches}
% \alison{this RQ should come before this (and be broken down into the specific RQs)}

\para{Task, data, and model.}
% \alison{briefly introduce the summarization task here, then talk about the two datasets and the model we implement}
The task is to read a document and summarize the document and each participant summarizes 10 documents.
Informal and formal writing might impact how a human understands the context and formulates the summary. 
We employ the Reddit-TIFU dataset \citep{kim2018abstractive} for informal writing and Extreme Summarization (XSum) dataset \citep{narayan2018don} for formal writing.
% As there are many instances in both datasets, 
We randomly selected 120 
% \ke{shouldn't the final size be 120?} 
instances from the default test set downloaded from Huggingface \footnote{\href{https://huggingface.co/datasets/reddit_tifu}{Reddit-TIFU}, \href{https://huggingface.co/datasets/xsum}{XSum}}.
% \ke{provide a link here}.
As lengthy documents make the task more difficult and short documents make the task easier, we selected instances which length fall between the 25th and 75th percentile.

\begin{table}[t]
    \small
    \centering
    \begin{tabular}{p{0.1\textwidth}p{0.15\textwidth}}
    \toprule
    \multicolumn{2}{c}{Rouge-1/Rouge-2/Rouge-L} \\
    Reddit & 27.99/9.81/22.94\\
    Xsum & 47.60/24.83/39.64 \\
    \bottomrule
    \end{tabular}
    \caption{Pegasus performance on Reddit and Xsum datasets.}
    \label{tb:pegasus_performance}
\end{table}
% \alison{provide more details on Pegasus; how well it works and for what types of data it has been used before; describe more details about pretraining}
% \alison{its not clear from this section what the model is doing; let's merge this with data and talk about the task (summarizing documents)}
We use the Pegasus model \cite{zhang2020pegasus} to generate summaries for the two datasets.
The base model is trained with stochastically sample important sentences and models for respective datasets are finetuned from it.
% The Pegasus model for respective dataset is then finetuned from the base model.
The performance of the models are stated in \tabref{tb:pegasus_performance}.
% To ensure the quality of the generated summaries, they are generated by the Pegasus \cite{zhang2020pegasus} model pretrained on the respective dataset, as provided by Huggingface.
% The same tokenizer is used for both datasets.

% \alison{I suppose we need to say this somewhere}
We built a web application to facilitate the first phase of the experiment and conducted a pilot study before running the full user study.
Read appendix for more details of pilot study.
% \footnote{The web application went through a few rounds of iteration to ensure that the wordings and flow was correct and easy to follow.We did two pilot study sessions, the first was conducted among researchers with 5 users mainly to get feedback on the usability of the web application and the average duration of a session, and the second one was conducted with actual targeted users on Upwork.} 



\para{Study design.}
% \alison{we actually did not use a 2x3. we did two 1x3 experiments (one for each dataset) where the only factor is assistance}
% \alison{we might move this to the intro and shorten if we we're having spaces issues}
The study used a 
% 1 x 3 
between-subjects experimental design, using \textit{AI assistance} as the factor.
% with factors of 
% --none, generated summary, reference-- 
% Given that there are two datasets, totalling to 6 conditions. 
The AI assistance factors are the following:
\begin{enumerate}
    \item \textbf{Manual}. There is no provided assistance.
    \item \textbf{Generated summary}. An AI-generated summary is provided as assistance.
    \item \textbf{Reference}. The ground truth summary provided by the dataset is provided as assistance.
\end{enumerate}
% --Xsum, Reddit-TIFU

% \alison{up to?}

% \subsection{Interface \& User study}
%\subsection{User study method}
% \alison{is this your study method section? perhaps rename}



\para{Participants.}
% \alison{be more specific about the skills we wanted and why we used upwork; talk about how much people were paid here and report on their gender, age, etc.}
We recruited 72 participants in total from the Upwork platform.\footnote{https://www.upwork.com}
% \alison{didn't we pay a bonus as well?} \viv{we didn't pay bonus}
Based on pilot studies, we anticipated the entire process would take 60 minutes and we paid participants \$20.
% \alison{oof we paid too much? does that average time count all the way from instruction to submitting the survey? also need to report standard deviation - we can report on this in the results or data and analysis section instead} \viv{time taken is measured from start till finish}
Each participant session took on average 34 minutes ($SD$=15)
% We used Upwork to recruit more motivated and experienced participants compared to other common crowdworking platforms.
% , such as Mechanical Turk. 
%the task of summarizing text requires certain set of skills and also to ensure certain level of summary quality, 
% Specifically, 
We used Upwork to recruit participants with experience in writing, journalism, or communication to ensure higher quality human-written summaries. 
% Participants were required to be a native or bilingual English speaker, have at least 90\% job success score and possess expertise in one or more of: writing, journalism, and communication.
Participants were asked two pre-task questions, 
% the first question was on 
their familiarity with Reddit and British culture.
% and the second question was on their familiarity with British news and culture.
% If participants answered that they have some experience, 
% assuming that they satisfy the previous criteria mentioned, 
% they would be hired as one of the participants.
Pre-task questions ensure that participants do not work on the task without \textit{any} knowledge of the domain.
% (i.e., Reddit and British news and)
% \alison{explain why we asked for reading test score: (1) selection criteria and (2) ensure similar average score per condition... you might need to describe how condition assignment happened somewhere...}
We also asked participants to report their reading test score based on a website \footnote{https://swiftread.com}.
The reading and comprehension test scores help to (1) eliminate potential participants who do not pay close attention to reading and (2) ensure similar average score per condition.
Lastly, participants were assigned to conditions in a round-robin manner.
% while adhering to similar average reading speed in different conditions.
% For instance, if a participant was assigned to manual in Reddit, the next participant would be assigned to generated summary in Reddit, etc.


% \alison{report the average age and standard deviation}
Participants' varied in age from 18 to 71 (M=32, SD=12) and gender (45 female, 22 male, 3 non-binary, 2 preferred not to disclose).

% \alison{did we ask any other pre-task or qualifying questions?}


% \para{Pilot study.}
% % \alison{this might fit better somewhere else; perhaps earlier?}
% \alison{maybe this is better as a footnote for saving space (you can footnote it when you first mention the pilot)}
% The web application went through a few rounds of iteration to ensure that the wordings and flow was correct and easy to follow.
% We did two pilot study sessions, the first was conducted among researchers with 5 users mainly to get feedback on the usability of the web application and the average duration of a session, and the second one was conducted with actual targeted users on Upwork.


% \para{User study flow.}
\para{Procedure.}
%From pilot studies, we anticipated it would take about an hour to complete the task.
An equal number of participants (36)
% \alison{how many?}
were randomly assigned to each dataset and summarization condition.
During the study, participants completed four phases: (1) instructions, (2) tutorial and practice, (3) summarization task, and (4) post-task survey.
% Participants were paid \$20.
%Using the web application to collect information, participants went through four phases during the study: (1) instructions; (2) tutorial and practice; (3) summarization task; (4) exit survey.
% \alison{is this your protocol section? perhaps rename}
% \alison{let's just very briefly discuss the instructions, tutorial and practice; the important part is the summarization task} \viv{ok sounds good}
During the \textit{tutorial and practice}, participants are taught the criteria of a good summary and how to write a good summary.
We used the same criteria of a good summary as in \citet{stiennon2020learning}.
The participants reviewed two randomly selected documents with a bad and good summary each with individual explanations provided.
% The two documents are randomly selected from the original training set of both Reddit and Xsum.
% Individual explanations are given for each summary provided.
Read appendix for details on each phase.
% \figref{fig:tutorial} shows the criteria of a good summary.



% During the \textit{practice} phase, participants applied what they learned in the tutorial phase and practiced how to write a good summary.
% To refrain from any confusion, the interface in the practice phase is exactly the same as the actual summarization task phase.
% Participants have access to the criteria as guidance.
% % \figref{fig:practice} shows the interface during the practice phase.
% After completing the summary, participants rated their agreement with two or three statements (depending on the assigned condition) about the task.
% % \alison{don't need to detail the measures here (they have their own section), just say they rated their agreement to three statements about the task.. except, how to explain that we don't report on one of these measures?}
% % \viv{can we just leave out the third one?}
% % \alison{yes, since we didn't log or report on it let's leave it off}
% We asked participants to rate their agreement for the following statements: (1) I found it difficult to understand the content of the document; (2) I found it difficult to summarize the document well. 
% % (3) The provided summary was of poor quality.
% % The last statement is only shown to participants who have provided summary or reference as AI assistance.
% % \ke{let's define clearly the conditions at the beginning, like (1) AI model automatically generated summary; (2) reference summary which is provided by dataset; (3) manual, where no summary as assistance provided}.

% During the actual summarization task phase, participants see the exact same interface as they saw in the practice phase.
% Finally, participants They would complete summarizing 10 documents and proceed to answer an exit survey.


% \para{Pilot study.}
% \alison{this might fit better somewhere else; perhaps earlier?}
% The web application went through a few rounds of iteration to ensure that the wordings and flow was correct and easy to follow.
% We did two pilot study sessions, the first was conducted among researchers with 5 users mainly to get feedback on the usability of the web application and the average duration of a session, and the second one was conducted with actual targeted users on Upwork.


\para{Measures.}
\label{para:measures}
% We report on summarization quality, efficiency, and user experience for the summarization task. 
% \alison{summary quality belongs in the second phase discussion but we can forward ref it here}
Summary quality is measured using human evaluation where a summary is rated on four axes: Coherence, Accuracy, Coverage, and Overall, on a scale of 1 to 7 
% (see \secref{sec:summary_evaluate}) 
and ROUGE.
% We also report on summary quality as measured by automatic measures (ROUGE), but such measures do not typically align well with human quality ratings~\cite{}.
%Summary quality is rated by four axes, Coherence, Accuracy, Coverage, and Overall on a 7-point scale from 1 to 7.
%We follow the rating design as written by \citet{stiennon2020learning}.
Efficiency is measured by the amount of time taken to complete writing a summary for each document. 
% As it is not simple to extract summarization time from reading time (as participants might switch back and forth between reading the original document and writing their summaries), we measure the time taken from when the participant receives the original document to when they submit their summary.
% We account for individual reading time differences by ensuring a similar average reading speed, measured by words per minute (WPM), between participants (M=358, SD=).
% \alison{we need to report on average reading score per condition somewhere - perhaps here? or report somewhere else and reference from here}
Finally, we report on three subjective measures related to user experience, collected using 7 point rating scales (from strongly disagree to strongly agree):
task-level task ease, or ``The summarization tasks were difficult.''; 
instance-level task ease, or ``I found it difficult to summarize the article well.''; and, task-level frustration, or ``Performing the summarization tasks was frustrating.''

==> sections/data_evaluation.tex <==
\subsection{Phase II: Human Evaluation of the Collected Summaries}
\label{sec:summary_evaluate}
% \alison{instead of saying what you will write about in this section, give an overview of the purpose of this Phase and what was done; you can also succinctly introduce the summary types (conditions) here instead of later.}
% In the previous section, we described the process of collecting human written summaries and in this section, we detail the process of evaluating the summaries collected.
% In the second phase of the experiment, 
We hire another set of participants to evaluate the human-written summaries.
% collected during the first phase of the experiment.
% A participant reads a news article or Reddit post and 
A participants evaluates six different summaries written or generated for the same document.
% \alison{might be more clear in a list? }
The six types of summaries are the following: 
\begin{enumerate}
    \item \textbf{Manual}. It was written without assistance.
    \item \textbf{Model-generated}. The provided summary is generated by the Pegasus model.
    \item \textbf{Reference}. The provided summary is from the original dataset.
    \item \textbf{Model-generated + post-edit}. It is written by a human who is shown a model-generated summary.
    \item \textbf{Reference + post-edit.} It is written by a human who is shown a reference summary.
    \item \textbf{Random.} It is generated by randomly selecting two sentences from another dataset. This summary helps to weed out turkers who do not pay attention. Refer to appendix for details.
    % For instance, if the participant sees a Reddit post, the \textit{Random} summary is a summary generated from a news article from the Xsum dataset.
\end{enumerate}

% \subsection{User study}
% \alison{this is not a user study; this is purely a data collecion task to evaluate the summaries collected in Phase I}
% \viv{what is a good subtitle?}


\para{Participants.}
% For the second phase of the experiment, as compared to writing a summary, evaluating a summary is an easier task.
We hire participants from crowdsourcing platform, Amazon Mechanical Turk as evaluating summaries is a relatively easier task.
To ensure quality responses, we only employ turkers who satisfy the following criteria: (1) completed 5000 HITs; (2) 97\% HIT approval rate; (3) Reside in the United States, Australia, and United Kingdom.
We allow duplicate participation given the assumption that users become better at the task if they constantly work on a similar task.
Refer to appendix on how we did quality-control on turkers.

\para{Procedure.}
The participant goes through two phases in this user study: (1) tutorial and attention check; and (2) the task of evaluating summaries.
A tutorial is written at the start of the task to teach the participant how to evaluate a summary.
We included an attention check open-ended question to ensure that the participant read through and understood the tutorial.
% Following \citet{stiennon2020learning}, a summary is rated on four axes: Coherence, Accuracy, Coverage, and Overall, on a scale of 1 to 7.
% Examples are given to ensure that the participant knows what a rating of 1, 4, or 7 look like.
% \figref{fig:rating_table} shows the table that was shown to participants.
To further solidify their understanding, we also included two examples with ratings and explanations.
% \figref{fig:evaluate_examples} shows the two examples taken from the training set of datasets.
Explanations are curated by the researchers and iterated a few times upon getting feedback.
% The attention check question does not disqualify the participant but only allow the participant to proceed to the actual task if only they answered it correctly.

% A participant reads a news article or Reddit post and evaluates six different summaries written for the same post.
% % \alison{might be more clear in a list? }
% The six types of summaries are the following: 
% \begin{enumerate}
%     \item \textbf{Manual}. The summary was written without any form of assistance.
%     \item \textbf{Model-generated}. The provided summary is generated by the Pegasus model.
%     \item \textbf{Reference}. The provided summary is from the original dataset.
%     \item \textbf{Model-generated + post-edit}. The summary is written by a participant who is shown a model-generated summary as provided assistance.
%     \item \textbf{Reference + post-edit} The summary is written by a participant who is shown a reference summary as provided assistance.
%     \item \textbf{Random} The summary is generated by randomly selecting two sentences from the opposite dataset.For instance, if the participant sees a Reddit post, the \textit{Random} summary is a summary generated from a news article from the Xsum dataset.
% \end{enumerate}
% (1) \textit{Manual} where the summary was written without any form of assistance; (2) \textit{Model-generated} summary that is generated by the Pegasus model; (3) \textit{Reference} that is provided with the original dataset; (4) \textit{Model-generated + post-edit} summary that is written by a participant who is shown a model-generated summary as provided assistance; (5) \textit{Reference + post-edit} summary that is written by a participant who is shown a reference summary as provided assistance; and (6) \textit{Random} summary that is generated by randomly selecting two sentences from the opposite dataset.


% \begin{figure}[t]
%   \centering
%     \centering
%     \includegraphics[width=.4\textwidth]{figs/sample-franklin.png}
%   \caption{This shows an example of a random summary for a particular instance from the Reddit-TIFU dataset.}
%   \label{fig:random_summary}
%   \Description{}
% \end{figure}

% \para{The purpose of the \textit{Random} summary.}
% The \textit{Random} summary helps to weed out turkers that do not pay attention and simply click through the rating scales.
% Since the order of the summaries is randomized, the \textit{Random} summary can appear in any position, minimizing the potential of participants not paying sufficient attention to details.
% Given that there are four axes to rating a summary, we eliminate and leave out responses of turkers who do not give a rating of 1 to Coverage and Accuracy.
% Since the \textit{Random} summary is created by using another document from an entirely different dataset, it is fair to assume that the content will not overlap and be inaccurate.
% \figref{fig:random_summary} shows an example of a random summary for post from the Reddit-TIFU article.


% \para{Eliminating the bad apples.}
% % \viv{this is one of our contributions. should we elaborate more on this?}\alison{if it will be a contribution, then yes}
% % \viv{let's discuss with joel}
% We deployed a total of 1200 evaluations (i.e., 120 HITs x 2 datasets x 5 samples) on Mechanical Turk.
% To maintain the integrity of the results, instead of deploying all assignments at once, we split the assignments into 10 batches.
% At the end of a batch deployment, turkers who failed the Random summary check will be blacklisted and not allowed to take accept future HITs in this group. A total of 113 workers completed the 1200 evaluations.


==> sections/study.tex <==
\section{Evaluating AI Assistance for Text Summarization}

We explored how providing summaries (whether from human or AI) for post-editing affects (RQ1) summary quality, (RQ2) efficiency, and (RQ3) user experience, compared to fully manual or fully automatic approaches.
% \joel{this text is very similar to the text in the preceding sentence} 

%To examine the effects of AI assistance and post-editing on the text summarization process, we focus on the following three research questions:
%\begin{enumerate}
%    \item \textbf{RQ1:} How does providing summaries (whether from human or AI) affect \textit{summary quality} compared to manual summarization and automatic summarization?
%    \item \textbf{RQ2:} How does providing summaries (whether from human or AI) affect \textit{efficiency}, as compared to manual summarization?
%    \item \textbf{RQ3:} How does providing summaries (whether from human or AI) affect \textit{user experience} compared to manual summarization?
%\end{enumerate}

\input{sections/method}
%\input{sections/results}
